A Wave is Worth 100 Words: Investigating Cross-Domain Transferability in Time Series

Time series analysis is a fundamental data mining task that supervised training methods based on empirical risk minimization have proven their effectiveness on specific tasks and datasets. However, the acquisition of well-annotated data is costly and a large amount of unlabeled series data is under-utilized. Due to distributional shifts across various domains and different patterns of interest across multiple tasks. The problem of cross-domain multi-task migration of time series remains a significant challenge. To address these problems, this paper proposes a novel cross-domain pretraining method based on Wave Quantization (termed as WQ4TS), which can be combined with any advanced time series model and applied to multiple downstream tasks. Specifically, we transfer the time series data from different domains into a common spectral latent space, and enable the model to learn the temporal pattern knowledge of different domains directly from the common space and utilize it for the inference of downstream tasks, thereby mitigating the challenge of heterogeneous cross-domains migration. The establishment of spectral latent space brings at least three benefits, cross-domain migration capability thus adapting to zero- and few-shot scenarios without relying on priori knowledge of the dataset, general compatible cross-domain migration framework without changing the existing model structure, and robust modeling capability thus achieving SOTA results in multiple downstream tasks. To demonstrate the effectiveness of the proposed approach, we conduct extensive experiments including three important tasks: forecasting, imputation, and classification. And three common real-world data scenarios are simulated: full-data, few-shot, and zero-shot. The proposed WQ4TS achieves the best performance on 87.5% of all tasks, and the average improvement of the metrics on all the tasks is up to 34.7%.

==> segments/7-Acknowledgements.tex <==
\section*{Acknowledgements}
This work was supported by the National Natural Science Foundation of China (71901011, U1811463, 51991391, 51991395, U21A20516).

==> tables/classification.tex <==
\begin{table*}[htbp]
  \caption{Classfication (full-data)}\label{tab:classification}
  \vskip 0.05in
  \centering
  \resizebox{1.99\columnwidth}{!}{
  \begin{threeparttable}
  \begin{small}
  \renewcommand{\multirowsetup}{\centering}
  \setlength{\tabcolsep}{1pt}
  \begin{tabular}{c|cccc|c||cccc|c||cccc|c||cccc|c}

    \midrule
    \midrule
    \multicolumn{1}{c}{\multirow{2}{*}{Models}} & 
    \multicolumn{5}{c}{\rotatebox{0}{\scalebox{0.8}{\textbf{CWTFormer}}}} &
    \multicolumn{5}{c}{\rotatebox{0}{\scalebox{0.8}{OneFitsAll}}} &
    \multicolumn{5}{c}{\rotatebox{0}{\scalebox{0.8}{PatchTST}}} &
    \multicolumn{5}{c}{\rotatebox{0}{\scalebox{0.8}{TimesNet}}} \\
    
    \multicolumn{1}{c}{} & 
    \multicolumn{5}{c}{\scalebox{0.8}{(\textbf{ours})}} & 
    \multicolumn{5}{c}{\scalebox{0.8}{\citeyearpar{Zhou2023OneFA}}} & 
    \multicolumn{5}{c}{\scalebox{0.8}{\citeyearpar{Nie2023ATS}}} & 
    \multicolumn{5}{c}{\scalebox{0.8}{\citeyearpar{wu2023timesnet}}} \\
    
    \cmidrule(lr){3-21}
    
    \multicolumn{1}{c}{Metric (\%)} & 
    \scalebox{0.78}{Acc} &\scalebox{0.78}{Pre} &\scalebox{0.78}{Rec} &\scalebox{0.78}{F1} &\scalebox{0.78}{Avg} & 
    \scalebox{0.78}{Acc} &\scalebox{0.78}{Pre} &\scalebox{0.78}{Rec} &\scalebox{0.78}{F1} &\scalebox{0.78}{Avg} & 
    \scalebox{0.78}{Acc} &\scalebox{0.78}{Pre} &\scalebox{0.78}{Rec} &\scalebox{0.78}{F1} &\scalebox{0.78}{Avg} & 
    \scalebox{0.78}{Acc} &\scalebox{0.78}{Pre} &\scalebox{0.78}{Rec} &\scalebox{0.78}{F1} &\scalebox{0.78}{Avg} \\
    
    \midrule
    
    \scalebox{0.78}{BeetleFly} &
    \scalebox{0.78}{80.00} &\scalebox{0.78}{80.00} &\scalebox{0.78}{80.00} &\scalebox{0.78}{80.00} &\scalebox{0.78}{80.00} &
    \scalebox{0.78}{85.00} &\scalebox{0.78}{88.46} &\scalebox{0.78}{85.00} &\scalebox{0.78}{84.65} &\scalebox{0.78}{85.78} &
    \scalebox{0.78}{85.00} &\scalebox{0.78}{88.46} &\scalebox{0.78}{85.00} &\scalebox{0.78}{84.65} &\scalebox{0.78}{85.78} &
    \scalebox{0.78}{75.00} &\scalebox{0.78}{83.33} &\scalebox{0.78}{75.00} &\scalebox{0.78}{73.33} &\scalebox{0.78}{76.66} \\
    
    \scalebox{0.78}{BirdChicken} &
    \scalebox{0.78}{65.00} &\scalebox{0.78}{65.15} &\scalebox{0.78}{65.00} &\scalebox{0.78}{64.91} &\scalebox{0.78}{65.01} &
    \scalebox{0.78}{75.00} &\scalebox{0.78}{75.25} &\scalebox{0.78}{75.00} &\scalebox{0.78}{74.94} &\scalebox{0.78}{75.05} &
    \scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &
    \scalebox{0.78}{65.00} &\scalebox{0.78}{79.41} &\scalebox{0.78}{65.00} &\scalebox{0.78}{60.11} &\scalebox{0.78}{67.38} \\
    
    \scalebox{0.78}{BME} &
    \scalebox{0.78}{96.00} &\scalebox{0.78}{96.43} &\scalebox{0.78}{96.00} &\scalebox{0.78}{96.02} &\scalebox{0.78}{96.11} &
    \scalebox{0.78}{93.33} &\scalebox{0.78}{93.53} &\scalebox{0.78}{93.33} &\scalebox{0.78}{93.35} &\scalebox{0.78}{93.39} &
    \scalebox{0.78}{88.00} &\scalebox{0.78}{91.18} &\scalebox{0.78}{88.00} &\scalebox{0.78}{88.32} &\scalebox{0.78}{88.88} &
    \scalebox{0.78}{92.67} &\scalebox{0.78}{93.99} &\scalebox{0.78}{92.67} &\scalebox{0.78}{92.66} &\scalebox{0.78}{93.00} \\
    
    \scalebox{0.78}{CBF} &
    \scalebox{0.78}{97.67} &\scalebox{0.78}{97.70} &\scalebox{0.78}{97.67} &\scalebox{0.78}{97.65} &\scalebox{0.78}{97.67} &
    \scalebox{0.78}{87.67} &\scalebox{0.78}{89.96} &\scalebox{0.78}{87.66} &\scalebox{0.78}{87.57} &\scalebox{0.78}{88.22} &
    \scalebox{0.78}{89.78} &\scalebox{0.78}{89.94} &\scalebox{0.78}{89.81} &\scalebox{0.78}{89.84} &\scalebox{0.78}{89.84} &
    \scalebox{0.78}{93.67} &\scalebox{0.78}{93.68} &\scalebox{0.78}{93.68} &\scalebox{0.78}{93.67} &\scalebox{0.78}{93.67} \\
        
    \scalebox{0.78}{Chinatown} &
    \scalebox{0.78}{98.96} &\scalebox{0.78}{98.02} &\scalebox{0.78}{98.93} &\scalebox{0.78}{98.46} &\scalebox{0.78}{98.59} &
    \scalebox{0.78}{96.79} &\scalebox{0.78}{94.94} &\scalebox{0.78}{97.46} &\scalebox{0.78}{96.08} &\scalebox{0.78}{96.32} &
    \scalebox{0.78}{95.63} &\scalebox{0.78}{94.38} &\scalebox{0.78}{94.67} &\scalebox{0.78}{94.52} &\scalebox{0.78}{94.80} &
    \scalebox{0.78}{97.96} &\scalebox{0.78}{96.53} &\scalebox{0.78}{98.59} &\scalebox{0.78}{97.49} &\scalebox{0.78}{97.64} \\
    
    \scalebox{0.78}{ChlorineConcentration} &
    \scalebox{0.78}{53.26} &\scalebox{0.78}{17.75} &\scalebox{0.78}{33.33} &\scalebox{0.78}{23.17} &\scalebox{0.78}{31.88} &
    \scalebox{0.78}{60.05} &\scalebox{0.78}{65.30} &\scalebox{0.78}{46.19} &\scalebox{0.78}{46.64} &\scalebox{0.78}{54.55} &
    \scalebox{0.78}{57.24} &\scalebox{0.78}{51.82} &\scalebox{0.78}{39.09} &\scalebox{0.78}{33.60} &\scalebox{0.78}{45.44} &
    \scalebox{0.78}{53.75} &\scalebox{0.78}{51.17} &\scalebox{0.78}{34.05} &\scalebox{0.78}{24.64} &\scalebox{0.78}{40.90} \\
    
    \scalebox{0.78}{CricketX} &
    \scalebox{0.78}{16.41} &\scalebox{0.78}{7.62} &\scalebox{0.78}{17.46} &\scalebox{0.78}{10.06} &\scalebox{0.78}{12.89} &
    \scalebox{0.78}{60.77} &\scalebox{0.78}{66.36} &\scalebox{0.78}{61.52} &\scalebox{0.78}{62.31} &\scalebox{0.78}{62.74} &
    \scalebox{0.78}{67.69} &\scalebox{0.78}{68.66} &\scalebox{0.78}{68.24} &\scalebox{0.78}{68.17} &\scalebox{0.78}{68.19} &
    \scalebox{0.78}{60.26} &\scalebox{0.78}{60.14} &\scalebox{0.78}{61.06} &\scalebox{0.78}{59.95} &\scalebox{0.78}{60.35} \\
    
    \scalebox{0.78}{CricketY} &
    \scalebox{0.78}{13.08} &\scalebox{0.78}{2.81} &\scalebox{0.78}{12.40} &\scalebox{0.78}{4.50} &\scalebox{0.78}{8.20} &
    \scalebox{0.78}{64.10} &\scalebox{0.78}{67.36} &\scalebox{0.78}{64.00} &\scalebox{0.78}{65.05} &\scalebox{0.78}{65.13} &
    \scalebox{0.78}{65.38} &\scalebox{0.78}{68.78} &\scalebox{0.78}{65.73} &\scalebox{0.78}{66.55} &\scalebox{0.78}{66.61} &
    \scalebox{0.78}{65.38} &\scalebox{0.78}{67.00} &\scalebox{0.78}{65.41} &\scalebox{0.78}{65.72} &\scalebox{0.78}{65.88} \\
        
    \scalebox{0.78}{CricketZ} &
    \scalebox{0.78}{9.23} &\scalebox{0.78}{0.77} &\scalebox{0.78}{8.33} &\scalebox{0.78}{1.41} &\scalebox{0.78}{4.93} &
    \scalebox{0.78}{62.82} &\scalebox{0.78}{65.25} &\scalebox{0.78}{62.40} &\scalebox{0.78}{62.73} &\scalebox{0.78}{63.30} &
    \scalebox{0.78}{68.97} &\scalebox{0.78}{68.57} &\scalebox{0.78}{67.76} &\scalebox{0.78}{67.81} &\scalebox{0.78}{68.28} &
    \scalebox{0.78}{58.46} &\scalebox{0.78}{58.23} &\scalebox{0.78}{57.29} &\scalebox{0.78}{57.17} &\scalebox{0.78}{57.79} \\
    
    \scalebox{0.78}{DistalPhalanxOutlineAgeGroup} &
    \scalebox{0.78}{68.35} &\scalebox{0.78}{50.86} &\scalebox{0.78}{51.69} &\scalebox{0.78}{48.18} &\scalebox{0.78}{54.77} &
    \scalebox{0.78}{73.38} &\scalebox{0.78}{79.31} &\scalebox{0.78}{68.90} &\scalebox{0.78}{70.69} &\scalebox{0.78}{73.07} &
    \scalebox{0.78}{74.82} &\scalebox{0.78}{79.76} &\scalebox{0.78}{76.66} &\scalebox{0.78}{75.97} &\scalebox{0.78}{76.80} &
    \scalebox{0.78}{76.26} &\scalebox{0.78}{78.12} &\scalebox{0.78}{75.77} &\scalebox{0.78}{76.21} &\scalebox{0.78}{76.59} \\
    
    \scalebox{0.78}{DistalPhalanxOutlineCorrect} &
    \scalebox{0.78}{58.33} &\scalebox{0.78}{29.17} &\scalebox{0.78}{50.00} &\scalebox{0.78}{36.84} &\scalebox{0.78}{43.59} &
    \scalebox{0.78}{74.28} &\scalebox{0.78}{77.38} &\scalebox{0.78}{70.50} &\scalebox{0.78}{70.82} &\scalebox{0.78}{73.25} &
    \scalebox{0.78}{71.74} &\scalebox{0.78}{72.44} &\scalebox{0.78}{68.57} &\scalebox{0.78}{68.85} &\scalebox{0.78}{70.40} &
    \scalebox{0.78}{76.45} &\scalebox{0.78}{75.78} &\scalebox{0.78}{75.96} &\scalebox{0.78}{75.86} &\scalebox{0.78}{76.01} \\
    
    \scalebox{0.78}{DistalPhalanxTW} &
    \scalebox{0.78}{81.22} &\scalebox{0.78}{65.75} &\scalebox{0.78}{66.69} &\scalebox{0.78}{65.02} &\scalebox{0.78}{69.67} &
    \scalebox{0.78}{71.94} &\scalebox{0.78}{67.91} &\scalebox{0.78}{57.61} &\scalebox{0.78}{55.68} &\scalebox{0.78}{63.28} &
    \scalebox{0.78}{70.50} &\scalebox{0.78}{46.09} &\scalebox{0.78}{50.37} &\scalebox{0.78}{46.70} &\scalebox{0.78}{53.42} &
    \scalebox{0.78}{73.38} &\scalebox{0.78}{67.09} &\scalebox{0.78}{59.13} &\scalebox{0.78}{59.70} &\scalebox{0.78}{64.83} \\
        
    \scalebox{0.78}{Earthquakes} &
    \scalebox{0.78}{74.82} &\scalebox{0.78}{37.41} &\scalebox{0.78}{50.00} &\scalebox{0.78}{42.80} &\scalebox{0.78}{51.26} &
    \scalebox{0.78}{75.54} &\scalebox{0.78}{68.06} &\scalebox{0.78}{53.32} &\scalebox{0.78}{50.36} &\scalebox{0.78}{61.82} &
    \scalebox{0.78}{75.54} &\scalebox{0.78}{71.20} &\scalebox{0.78}{52.38} &\scalebox{0.78}{48.18} &\scalebox{0.78}{61.83} &
    \scalebox{0.78}{74.82} &\scalebox{0.78}{63.58} &\scalebox{0.78}{55.69} &\scalebox{0.78}{55.19} &\scalebox{0.78}{62.32} \\
    
    \scalebox{0.78}{ECG200} &
    \scalebox{0.78}{96.00} &\scalebox{0.78}{94.92} &\scalebox{0.78}{95.37} &\scalebox{0.78}{95.14} &\scalebox{0.78}{95.36} &
    \scalebox{0.78}{91.00} &\scalebox{0.78}{90.44} &\scalebox{0.78}{89.93} &\scalebox{0.78}{90.17} &\scalebox{0.78}{90.38} &
    \scalebox{0.78}{86.00} &\scalebox{0.78}{85.12} &\scalebox{0.78}{84.20} &\scalebox{0.78}{84.62} &\scalebox{0.78}{84.98} &
    \scalebox{0.78}{89.00} &\scalebox{0.78}{88.72} &\scalebox{0.78}{87.15} &\scalebox{0.78}{87.83} &\scalebox{0.78}{88.17} \\
    
    \scalebox{0.78}{ECG5000} &
    \scalebox{0.78}{95.53} &\scalebox{0.78}{79.79} &\scalebox{0.78}{65.63} &\scalebox{0.78}{71.76} &\scalebox{0.78}{77.93} &
    \scalebox{0.78}{94.56} &\scalebox{0.78}{76.62} &\scalebox{0.78}{56.73} &\scalebox{0.78}{62.01} &\scalebox{0.78}{72.48} &
    \scalebox{0.78}{94.67} &\scalebox{0.78}{73.41} &\scalebox{0.78}{56.40} &\scalebox{0.78}{59.97} &\scalebox{0.78}{71.11} &
    \scalebox{0.78}{93.93} &\scalebox{0.78}{77.58} &\scalebox{0.78}{55.31} &\scalebox{0.78}{60.50} &\scalebox{0.78}{71.83} \\
    
    \scalebox{0.78}{ElectricDevices} &
    \scalebox{0.78}{74.24} &\scalebox{0.78}{68.21} &\scalebox{0.78}{63.80} &\scalebox{0.78}{64.86} &\scalebox{0.78}{67.78} &
    \scalebox{0.78}{62.05} &\scalebox{0.78}{58.84} &\scalebox{0.78}{54.35} &\scalebox{0.78}{55.22} &\scalebox{0.78}{57.62} &
    \scalebox{0.78}{66.76} &\scalebox{0.78}{63.03} &\scalebox{0.78}{59.51} &\scalebox{0.78}{60.60} &\scalebox{0.78}{62.47} &
    \scalebox{0.78}{69.23} &\scalebox{0.78}{65.60} &\scalebox{0.78}{63.30} &\scalebox{0.78}{63.79} &\scalebox{0.78}{65.48} \\
        
    \scalebox{0.78}{EOGHorizontalSignal} &
    \scalebox{0.78}{8.29} &\scalebox{0.78}{0.69} &\scalebox{0.78}{8.33} &\scalebox{0.78}{1.28} &\scalebox{0.78}{4.65} &
    \scalebox{0.78}{42.27} &\scalebox{0.78}{43.44} &\scalebox{0.78}{42.40} &\scalebox{0.78}{41.23} &\scalebox{0.78}{42.34} &
    \scalebox{0.78}{51.38} &\scalebox{0.78}{52.18} &\scalebox{0.78}{51.36} &\scalebox{0.78}{51.09} &\scalebox{0.78}{51.50} &
    \scalebox{0.78}{34.25} &\scalebox{0.78}{35.02} &\scalebox{0.78}{34.12} &\scalebox{0.78}{29.72} &\scalebox{0.78}{33.28} \\
    
    \scalebox{0.78}{EOGVerticalSignal} &
    \scalebox{0.78}{8.29} &\scalebox{0.78}{0.69} &\scalebox{0.78}{8.33} &\scalebox{0.78}{1.28} &\scalebox{0.78}{4.65} &
    \scalebox{0.78}{35.08} &\scalebox{0.78}{32.81} &\scalebox{0.78}{34.92} &\scalebox{0.78}{31.87} &\scalebox{0.78}{33.67} &
    \scalebox{0.78}{47.51} &\scalebox{0.78}{41.46} &\scalebox{0.78}{47.55} &\scalebox{0.78}{43.53} &\scalebox{0.78}{45.01} &
    \scalebox{0.78}{27.62} &\scalebox{0.78}{26.05} &\scalebox{0.78}{27.39} &\scalebox{0.78}{25.10} &\scalebox{0.78}{26.54} \\
    
    \scalebox{0.78}{FaceAll} &
    \scalebox{0.78}{80.00} &\scalebox{0.78}{83.12} &\scalebox{0.78}{88.58} &\scalebox{0.78}{82.70} &\scalebox{0.78}{83.60} &
    \scalebox{0.78}{75.74} &\scalebox{0.78}{81.52} &\scalebox{0.78}{84.35} &\scalebox{0.78}{78.95} &\scalebox{0.78}{80.14} &
    \scalebox{0.78}{75.44} &\scalebox{0.78}{77.58} &\scalebox{0.78}{84.92} &\scalebox{0.78}{76.88} &\scalebox{0.78}{78.70} &
    \scalebox{0.78}{75.09} &\scalebox{0.78}{80.77} &\scalebox{0.78}{85.56} &\scalebox{0.78}{78.92} &\scalebox{0.78}{80.09} \\
    
    \scalebox{0.78}{FaceFour} &
    \scalebox{0.78}{84.09} &\scalebox{0.78}{83.21} &\scalebox{0.78}{84.84} &\scalebox{0.78}{83.63} &\scalebox{0.78}{83.94} &
    \scalebox{0.78}{90.91} &\scalebox{0.78}{91.04} &\scalebox{0.78}{91.13} &\scalebox{0.78}{90.92} &\scalebox{0.78}{91.00} &
    \scalebox{0.78}{85.23} &\scalebox{0.78}{86.53} &\scalebox{0.78}{85.98} &\scalebox{0.78}{86.13} &\scalebox{0.78}{85.97} &
    \scalebox{0.78}{89.77} &\scalebox{0.78}{90.20} &\scalebox{0.78}{90.17} &\scalebox{0.78}{90.11} &\scalebox{0.78}{90.06} \\
        
    \scalebox{0.78}{FacesUCR} &
    \scalebox{0.78}{95.51} &\scalebox{0.78}{94.50} &\scalebox{0.78}{92.51} &\scalebox{0.78}{93.06} &\scalebox{0.78}{93.89} &
    \scalebox{0.78}{86.15} &\scalebox{0.78}{86.55} &\scalebox{0.78}{82.36} &\scalebox{0.78}{83.67} &\scalebox{0.78}{84.68} &
    \scalebox{0.78}{84.83} &\scalebox{0.78}{85.28} &\scalebox{0.78}{80.03} &\scalebox{0.78}{81.78} &\scalebox{0.78}{82.98} &
    \scalebox{0.78}{85.07} &\scalebox{0.78}{85.94} &\scalebox{0.78}{82.21} &\scalebox{0.78}{83.44} &\scalebox{0.78}{84.17} \\
    
    \scalebox{0.78}{FiftyWords} &
    \scalebox{0.78}{80.77} &\scalebox{0.78}{66.02} &\scalebox{0.78}{66.52} &\scalebox{0.78}{64.08} &\scalebox{0.78}{69.35} &
    \scalebox{0.78}{70.33} &\scalebox{0.78}{60.85} &\scalebox{0.78}{55.43} &\scalebox{0.78}{55.19} &\scalebox{0.78}{60.45} &
    \scalebox{0.78}{75.16} &\scalebox{0.78}{65.69} &\scalebox{0.78}{60.40} &\scalebox{0.78}{59.12} &\scalebox{0.78}{65.09} &
    \scalebox{0.78}{66.15} &\scalebox{0.78}{54.22} &\scalebox{0.78}{48.47} &\scalebox{0.78}{47.80} &\scalebox{0.78}{54.16} \\
    
    \scalebox{0.78}{Fungi} &
    \scalebox{0.78}{87.63} &\scalebox{0.78}{91.46} &\scalebox{0.78}{87.14} &\scalebox{0.78}{83.95} &\scalebox{0.78}{87.54} &
    \scalebox{0.78}{86.56} &\scalebox{0.78}{90.73} &\scalebox{0.78}{87.83} &\scalebox{0.78}{86.14} &\scalebox{0.78}{87.81} &
    \scalebox{0.78}{94.62} &\scalebox{0.78}{95.00} &\scalebox{0.78}{94.37} &\scalebox{0.78}{93.24} &\scalebox{0.78}{94.31} &
    \scalebox{0.78}{85.48} &\scalebox{0.78}{86.36} &\scalebox{0.78}{86.68} &\scalebox{0.78}{85.75} &\scalebox{0.78}{86.07} \\
    
    \scalebox{0.78}{GunPointAgeSpan} &
    \scalebox{0.78}{96.14} &\scalebox{0.78}{96.86} &\scalebox{0.78}{96.06} &\scalebox{0.78}{96.09} &\scalebox{0.78}{96.29} &
    \scalebox{0.78}{89.56} &\scalebox{0.78}{90.06} &\scalebox{0.78}{89.49} &\scalebox{0.78}{89.51} &\scalebox{0.78}{89.66} &
    \scalebox{0.78}{89.24} &\scalebox{0.78}{89.80} &\scalebox{0.78}{89.17} &\scalebox{0.78}{89.19} &\scalebox{0.78}{89.35} &
    \scalebox{0.78}{94.94} &\scalebox{0.78}{94.94} &\scalebox{0.78}{94.94} &\scalebox{0.78}{94.94} &\scalebox{0.78}{94.94} \\
        
    \scalebox{0.78}{GunPointMaleVersusFemale} &
    \scalebox{0.78}{99.68} &\scalebox{0.78}{99.70} &\scalebox{0.78}{99.67} &\scalebox{0.78}{99.68} &\scalebox{0.78}{99.68} &
    \scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &
    \scalebox{0.78}{97.47} &\scalebox{0.78}{97.44} &\scalebox{0.78}{97.49} &\scalebox{0.78}{97.46} &\scalebox{0.78}{97.47} &
    \scalebox{0.78}{99.05} &\scalebox{0.78}{99.07} &\scalebox{0.78}{99.03} &\scalebox{0.78}{99.05} &\scalebox{0.78}{99.05} \\
    
    \scalebox{0.78}{GunPointOldVersusYoung} &
    \scalebox{0.78}{98.10} &\scalebox{0.78}{98.18} &\scalebox{0.78}{98.03} &\scalebox{0.78}{98.09} &\scalebox{0.78}{98.10} &
    \scalebox{0.78}{95.05} &\scalebox{0.78}{95.06} &\scalebox{0.78}{95.03} &\scalebox{0.78}{95.05} &\scalebox{0.78}{95.05} &
    \scalebox{0.78}{93.65} &\scalebox{0.78}{93.77} &\scalebox{0.78}{93.55} &\scalebox{0.78}{93.62} &\scalebox{0.78}{93.65} &
    \scalebox{0.78}{52.38} &\scalebox{0.78}{26.19} &\scalebox{0.78}{50.00} &\scalebox{0.78}{34.38} &\scalebox{0.78}{40.74} \\
    
    \scalebox{0.78}{GunPoint} &
    \scalebox{0.78}{96.00} &\scalebox{0.78}{96.05} &\scalebox{0.78}{95.98} &\scalebox{0.78}{96.00} &\scalebox{0.78}{96.01} &
    \scalebox{0.78}{92.67} &\scalebox{0.78}{93.09} &\scalebox{0.78}{92.60} &\scalebox{0.78}{92.64} &\scalebox{0.78}{92.75} &
    \scalebox{0.78}{76.00} &\scalebox{0.78}{78.47} &\scalebox{0.78}{75.80} &\scalebox{0.78}{75.37} &\scalebox{0.78}{76.41} &
    \scalebox{0.78}{94.00} &\scalebox{0.78}{94.23} &\scalebox{0.78}{93.95} &\scalebox{0.78}{93.99} &\scalebox{0.78}{94.04} \\
    
    \scalebox{0.78}{HouseTwenty} &
    \scalebox{0.78}{64.71} &\scalebox{0.78}{69.05} &\scalebox{0.78}{59.10} &\scalebox{0.78}{55.97} &\scalebox{0.78}{62.21} &
    \scalebox{0.78}{64.71} &\scalebox{0.78}{63.82} &\scalebox{0.78}{61.58} &\scalebox{0.78}{61.36} &\scalebox{0.78}{62.87} &
    \scalebox{0.78}{85.71} &\scalebox{0.78}{85.29} &\scalebox{0.78}{85.48} &\scalebox{0.78}{85.38} &\scalebox{0.78}{85.47} &
    \scalebox{0.78}{63.87} &\scalebox{0.78}{64.97} &\scalebox{0.78}{58.93} &\scalebox{0.78}{56.84} &\scalebox{0.78}{61.15} \\
        
    \scalebox{0.78}{InsectEPGRegularTrain} &
    \scalebox{0.78}{47.39} &\scalebox{0.78}{15.80} &\scalebox{0.78}{33.33} &\scalebox{0.78}{21.44} &\scalebox{0.78}{29.49} &
    \scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &
    \scalebox{0.78}{83.13} &\scalebox{0.78}{84.74} &\scalebox{0.78}{71.74} &\scalebox{0.78}{72.78} &\scalebox{0.78}{78.10} &
    \scalebox{0.78}{83.03} &\scalebox{0.78}{84.46} &\scalebox{0.78}{76.61} &\scalebox{0.78}{73.89} &\scalebox{0.78}{79.50} \\
    
    \scalebox{0.78}{InsectEPGSmallTrain} &
    \scalebox{0.78}{83.13} &\scalebox{0.78}{57.92} &\scalebox{0.78}{66.67} &\scalebox{0.78}{61.63} &\scalebox{0.78}{67.34} &
    \scalebox{0.78}{75.17} &\scalebox{0.78}{75.57} &\scalebox{0.78}{70.97} &\scalebox{0.78}{72.70} &\scalebox{0.78}{73.60} &
    \scalebox{0.78}{83.53} &\scalebox{0.78}{83.97} &\scalebox{0.78}{78.86} &\scalebox{0.78}{80.78} &\scalebox{0.78}{81.78} &
    \scalebox{0.78}{83.03} &\scalebox{0.78}{84.46} &\scalebox{0.78}{76.61} &\scalebox{0.78}{73.89} &\scalebox{0.78}{79.50} \\
    
    \scalebox{0.78}{InsectWingbeatSound} &
    \scalebox{0.78}{69.34} &\scalebox{0.78}{69.60} &\scalebox{0.78}{69.34} &\scalebox{0.78}{69.04} &\scalebox{0.78}{69.33} &
    \scalebox{0.78}{63.03} &\scalebox{0.78}{64.37} &\scalebox{0.78}{63.03} &\scalebox{0.78}{63.18} &\scalebox{0.78}{63.40} &
    \scalebox{0.78}{65.56} &\scalebox{0.78}{65.37} &\scalebox{0.78}{65.56} &\scalebox{0.78}{64.94} &\scalebox{0.78}{65.36} &
    \scalebox{0.78}{62.58} &\scalebox{0.78}{62.85} &\scalebox{0.78}{62.58} &\scalebox{0.78}{62.47} &\scalebox{0.78}{62.62} \\
    
    \scalebox{0.78}{ItalyPowerDemand} &
    \scalebox{0.78}{96.60} &\scalebox{0.78}{96.60} &\scalebox{0.78}{96.60} &\scalebox{0.78}{96.60} &\scalebox{0.78}{96.60} &
    \scalebox{0.78}{96.99} &\scalebox{0.78}{96.99} &\scalebox{0.78}{96.99} &\scalebox{0.78}{96.99} &\scalebox{0.78}{96.99} &
    \scalebox{0.78}{96.60} &\scalebox{0.78}{96.62} &\scalebox{0.78}{96.60} &\scalebox{0.78}{96.60} &\scalebox{0.78}{96.60} &
    \scalebox{0.78}{97.18} &\scalebox{0.78}{97.18} &\scalebox{0.78}{97.18} &\scalebox{0.78}{97.18} &\scalebox{0.78}{97.18} \\
        
    \scalebox{0.78}{Lightning7} &
    \scalebox{0.78}{53.42} &\scalebox{0.78}{31.01} &\scalebox{0.78}{43.43} &\scalebox{0.78}{35.67} &\scalebox{0.78}{40.88} &
    \scalebox{0.78}{76.71} &\scalebox{0.78}{83.73} &\scalebox{0.78}{76.43} &\scalebox{0.78}{74.16} &\scalebox{0.78}{77.76} &
    \scalebox{0.78}{71.23} &\scalebox{0.78}{71.52} &\scalebox{0.78}{69.87} &\scalebox{0.78}{66.31} &\scalebox{0.78}{69.73} &
    \scalebox{0.78}{76.71} &\scalebox{0.78}{77.11} &\scalebox{0.78}{78.09} &\scalebox{0.78}{75.81} &\scalebox{0.78}{76.93} \\
    
    \scalebox{0.78}{MedicalImages} &
    \scalebox{0.78}{84.47} &\scalebox{0.78}{81.67} &\scalebox{0.78}{76.79} &\scalebox{0.78}{77.84} &\scalebox{0.78}{80.19} &
    \scalebox{0.78}{70.53} &\scalebox{0.78}{66.96} &\scalebox{0.78}{66.78} &\scalebox{0.78}{65.50} &\scalebox{0.78}{67.44} &
    \scalebox{0.78}{68.55} &\scalebox{0.78}{65.34} &\scalebox{0.78}{60.71} &\scalebox{0.78}{61.11} &\scalebox{0.78}{63.93} &
    \scalebox{0.78}{73.03} &\scalebox{0.78}{68.97} &\scalebox{0.78}{63.52} &\scalebox{0.78}{65.37} &\scalebox{0.78}{67.72} \\
    
    \scalebox{0.78}{MiddlePhalanxOutlineAgeGroup} &
    \scalebox{0.78}{18.83} &\scalebox{0.78}{6.28} &\scalebox{0.78}{33.33} &\scalebox{0.78}{10.56} &\scalebox{0.78}{17.25} &
    \scalebox{0.78}{64.29} &\scalebox{0.78}{72.26} &\scalebox{0.78}{47.59} &\scalebox{0.78}{49.46} &\scalebox{0.78}{58.40} &
    \scalebox{0.78}{65.58} &\scalebox{0.78}{72.43} &\scalebox{0.78}{49.12} &\scalebox{0.78}{51.37} &\scalebox{0.78}{59.62} &
    \scalebox{0.78}{66.23} &\scalebox{0.78}{75.40} &\scalebox{0.78}{48.98} &\scalebox{0.78}{51.02} &\scalebox{0.78}{60.41} \\
    
    \scalebox{0.78}{MiddlePhalanxOutlineCorrect} &
    \scalebox{0.78}{57.04} &\scalebox{0.78}{28.52} &\scalebox{0.78}{50.00} &\scalebox{0.78}{36.32} &\scalebox{0.78}{42.97} &
    \scalebox{0.78}{61.86} &\scalebox{0.78}{68.65} &\scalebox{0.78}{56.19} &\scalebox{0.78}{50.37} &\scalebox{0.78}{59.27} &
    \scalebox{0.78}{58.42} &\scalebox{0.78}{62.37} &\scalebox{0.78}{52.00} &\scalebox{0.78}{42.24} &\scalebox{0.78}{53.76} &
    \scalebox{0.78}{85.57} &\scalebox{0.78}{86.07} &\scalebox{0.78}{84.48} &\scalebox{0.78}{84.99} &\scalebox{0.78}{85.28} \\
    
    \scalebox{0.78}{MiddlePhalanxTW} &
    \scalebox{0.78}{70.39} &\scalebox{0.78}{41.28} &\scalebox{0.78}{51.17} &\scalebox{0.78}{45.12} &\scalebox{0.78}{51.99} &
    \scalebox{0.78}{60.39} &\scalebox{0.78}{42.11} &\scalebox{0.78}{38.75} &\scalebox{0.78}{35.71} &\scalebox{0.78}{44.24} &
    \scalebox{0.78}{62.34} &\scalebox{0.78}{48.47} &\scalebox{0.78}{40.17} &\scalebox{0.78}{37.42} &\scalebox{0.78}{47.10} &
    \scalebox{0.78}{61.69} &\scalebox{0.78}{41.98} &\scalebox{0.78}{40.95} &\scalebox{0.78}{38.48} &\scalebox{0.78}{45.77} \\
    
    \scalebox{0.78}{MoteStrain} &
    \scalebox{0.78}{88.10} &\scalebox{0.78}{88.24} &\scalebox{0.78}{87.82} &\scalebox{0.78}{87.97} &\scalebox{0.78}{88.03} &
    \scalebox{0.78}{87.62} &\scalebox{0.78}{87.80} &\scalebox{0.78}{87.31} &\scalebox{0.78}{87.47} &\scalebox{0.78}{87.55} &
    \scalebox{0.78}{85.22} &\scalebox{0.78}{85.73} &\scalebox{0.78}{84.71} &\scalebox{0.78}{84.96} &\scalebox{0.78}{85.16} &
    \scalebox{0.78}{89.54} &\scalebox{0.78}{89.65} &\scalebox{0.78}{89.30} &\scalebox{0.78}{89.43} &\scalebox{0.78}{89.48} \\
    
    \scalebox{0.78}{PigAirwayPressure} &
    \scalebox{0.78}{1.92} &\scalebox{0.78}{0.04} &\scalebox{0.78}{1.92} &\scalebox{0.78}{0.07} &\scalebox{0.78}{0.99} &
    \scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &
    \scalebox{0.78}{4.81} &\scalebox{0.78}{4.09} &\scalebox{0.78}{4.81} &\scalebox{0.78}{4.11} &\scalebox{0.78}{4.45} &
    \scalebox{0.78}{10.58} &\scalebox{0.78}{9.69} &\scalebox{0.78}{10.58} &\scalebox{0.78}{9.21} &\scalebox{0.78}{10.02} \\
    
    \scalebox{0.78}{PigArtPressure} &
    \scalebox{0.78}{1.92} &\scalebox{0.78}{0.04} &\scalebox{0.78}{1.92} &\scalebox{0.78}{0.07} &\scalebox{0.78}{0.99} &
    \scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &
    \scalebox{0.78}{12.98} &\scalebox{0.78}{11.19} &\scalebox{0.78}{12.98} &\scalebox{0.78}{10.68} &\scalebox{0.78}{11.96} &
    \scalebox{0.78}{11.06} &\scalebox{0.78}{2.30} &\scalebox{0.78}{11.06} &\scalebox{0.78}{3.60} &\scalebox{0.78}{7.01} \\
        
    \scalebox{0.78}{PigCVP} &
    \scalebox{0.78}{1.92} &\scalebox{0.78}{0.04} &\scalebox{0.78}{1.92} &\scalebox{0.78}{0.07} &\scalebox{0.78}{0.99} &
    \scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &
    \scalebox{0.78}{7.21} &\scalebox{0.78}{8.17} &\scalebox{0.78}{7.21} &\scalebox{0.78}{6.97} &\scalebox{0.78}{7.39} &
    \scalebox{0.78}{9.62} &\scalebox{0.78}{7.88} &\scalebox{0.78}{9.62} &\scalebox{0.78}{6.15} &\scalebox{0.78}{8.32} \\
    
    \scalebox{0.78}{Plane} &
    \scalebox{0.78}{99.05} &\scalebox{0.78}{99.11} &\scalebox{0.78}{99.11} &\scalebox{0.78}{99.08} &\scalebox{0.78}{99.09} &
    \scalebox{0.78}{99.05} &\scalebox{0.78}{99.16} &\scalebox{0.78}{99.05} &\scalebox{0.78}{99.07} &\scalebox{0.78}{99.08} &
    \scalebox{0.78}{98.10} &\scalebox{0.78}{98.01} &\scalebox{0.78}{98.15} &\scalebox{0.78}{98.04} &\scalebox{0.78}{98.08} &
    \scalebox{0.78}{99.05} &\scalebox{0.78}{99.16} &\scalebox{0.78}{99.05} &\scalebox{0.78}{99.07} &\scalebox{0.78}{99.08} \\
    
    \scalebox{0.78}{PowerCons} &
    \scalebox{0.78}{50.00} &\scalebox{0.78}{25.00} &\scalebox{0.78}{50.00} &\scalebox{0.78}{33.33} &\scalebox{0.78}{39.58} &
    \scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &
    \scalebox{0.78}{98.89} &\scalebox{0.78}{98.91} &\scalebox{0.78}{98.89} &\scalebox{0.78}{98.89} &\scalebox{0.78}{98.89} &
    \scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} \\
    
    \scalebox{0.78}{ProximalPhalanxOutlineAgeGroup} &
    \scalebox{0.78}{48.78} &\scalebox{0.78}{16.26} &\scalebox{0.78}{33.33} &\scalebox{0.78}{21.86} &\scalebox{0.78}{30.06} &
    \scalebox{0.78}{84.39} &\scalebox{0.78}{56.18} &\scalebox{0.78}{61.30} &\scalebox{0.78}{58.62} &\scalebox{0.78}{65.12} &
    \scalebox{0.78}{87.80} &\scalebox{0.78}{81.74} &\scalebox{0.78}{79.77} &\scalebox{0.78}{80.67} &\scalebox{0.78}{82.50} &
    \scalebox{0.78}{85.85} &\scalebox{0.78}{76.64} &\scalebox{0.78}{70.35} &\scalebox{0.78}{72.08} &\scalebox{0.78}{76.23} \\
        
    \scalebox{0.78}{ProximalPhalanxOutlineCorrect} &
    \scalebox{0.78}{68.38} &\scalebox{0.78}{34.19} &\scalebox{0.78}{50.00} &\scalebox{0.78}{40.61} &\scalebox{0.78}{48.30} &
    \scalebox{0.78}{79.73} &\scalebox{0.78}{76.60} &\scalebox{0.78}{76.12} &\scalebox{0.78}{76.35} &\scalebox{0.78}{77.20} &
    \scalebox{0.78}{78.35} &\scalebox{0.78}{76.20} &\scalebox{0.78}{71.02} &\scalebox{0.78}{72.52} &\scalebox{0.78}{74.52} &
    \scalebox{0.78}{85.22} &\scalebox{0.78}{88.80} &\scalebox{0.78}{77.51} &\scalebox{0.78}{80.43} &\scalebox{0.78}{82.99} \\
    
    \scalebox{0.78}{ProximalPhalanxTW} &
    \scalebox{0.78}{87.44} &\scalebox{0.78}{77.46} &\scalebox{0.78}{70.73} &\scalebox{0.78}{68.10} &\scalebox{0.78}{75.93} &
    \scalebox{0.78}{80.49} &\scalebox{0.78}{39.21} &\scalebox{0.78}{45.17} &\scalebox{0.78}{41.91} &\scalebox{0.78}{51.70} &
    \scalebox{0.78}{81.95} &\scalebox{0.78}{56.48} &\scalebox{0.78}{53.84} &\scalebox{0.78}{53.57} &\scalebox{0.78}{61.46} &
    \scalebox{0.78}{82.93} &\scalebox{0.78}{65.09} &\scalebox{0.78}{62.37} &\scalebox{0.78}{62.22} &\scalebox{0.78}{68.15} \\
    
    \scalebox{0.78}{ShapesAll} &
    \scalebox{0.78}{1.67} &\scalebox{0.78}{0.03} &\scalebox{0.78}{1.67} &\scalebox{0.78}{0.05} &\scalebox{0.78}{0.85} &
    \scalebox{0.78}{72.67} &\scalebox{0.78}{73.93} &\scalebox{0.78}{72.67} &\scalebox{0.78}{71.95} &\scalebox{0.78}{72.80} &
    \scalebox{0.78}{78.50} &\scalebox{0.78}{79.20} &\scalebox{0.78}{78.50} &\scalebox{0.78}{77.97} &\scalebox{0.78}{78.54} &
    \scalebox{0.78}{61.00} &\scalebox{0.78}{59.79} &\scalebox{0.78}{61.00} &\scalebox{0.78}{59.34} &\scalebox{0.78}{60.28} \\
    
    \scalebox{0.78}{SmoothSubspace} &
    \scalebox{0.78}{33.33} &\scalebox{0.78}{11.11} &\scalebox{0.78}{33.33} &\scalebox{0.78}{16.67} &\scalebox{0.78}{23.61} &
    \scalebox{0.78}{86.00} &\scalebox{0.78}{85.89} &\scalebox{0.78}{86.00} &\scalebox{0.78}{85.79} &\scalebox{0.78}{85.92} &
    \scalebox{0.78}{76.67} &\scalebox{0.78}{76.67} &\scalebox{0.78}{76.67} &\scalebox{0.78}{76.20} &\scalebox{0.78}{76.55} &
    \scalebox{0.78}{96.67} &\scalebox{0.78}{96.78} &\scalebox{0.78}{96.67} &\scalebox{0.78}{96.66} &\scalebox{0.78}{96.69} \\
        
    \scalebox{0.78}{SonyAIBORobotSurface1} &
    \scalebox{0.78}{84.19} &\scalebox{0.78}{84.76} &\scalebox{0.78}{85.34} &\scalebox{0.78}{84.17} &\scalebox{0.78}{84.61} &
    \scalebox{0.78}{79.37} &\scalebox{0.78}{82.30} &\scalebox{0.78}{81.49} &\scalebox{0.78}{79.34} &\scalebox{0.78}{80.62} &
    \scalebox{0.78}{69.55} &\scalebox{0.78}{76.90} &\scalebox{0.78}{72.89} &\scalebox{0.78}{69.00} &\scalebox{0.78}{72.08} &
    \scalebox{0.78}{76.37} &\scalebox{0.78}{76.62} &\scalebox{0.78}{77.14} &\scalebox{0.78}{76.30} &\scalebox{0.78}{76.61} \\
    
    \scalebox{0.78}{SonyAIBORobotSurface2} &
    \scalebox{0.78}{89.72} &\scalebox{0.78}{89.37} &\scalebox{0.78}{88.76} &\scalebox{0.78}{89.04} &\scalebox{0.78}{89.22} &
    \scalebox{0.78}{86.15} &\scalebox{0.78}{85.75} &\scalebox{0.78}{84.67} &\scalebox{0.78}{85.13} &\scalebox{0.78}{85.42} &
    \scalebox{0.78}{85.31} &\scalebox{0.78}{84.35} &\scalebox{0.78}{84.82} &\scalebox{0.78}{84.57} &\scalebox{0.78}{84.76} &
    \scalebox{0.78}{81.32} &\scalebox{0.78}{80.25} &\scalebox{0.78}{80.19} &\scalebox{0.78}{80.22} &\scalebox{0.78}{80.50} \\
    
    \scalebox{0.78}{SwedishLeaf} &
    \scalebox{0.78}{95.20} &\scalebox{0.78}{95.28} &\scalebox{0.78}{95.32} &\scalebox{0.78}{95.23} &\scalebox{0.78}{95.26} &
    \scalebox{0.78}{84.80} &\scalebox{0.78}{85.66} &\scalebox{0.78}{84.97} &\scalebox{0.78}{84.56} &\scalebox{0.78}{85.00} &
    \scalebox{0.78}{91.20} &\scalebox{0.78}{91.33} &\scalebox{0.78}{91.62} &\scalebox{0.78}{91.33} &\scalebox{0.78}{91.37} &
    \scalebox{0.78}{88.00} &\scalebox{0.78}{88.32} &\scalebox{0.78}{88.43} &\scalebox{0.78}{87.90} &\scalebox{0.78}{88.16} \\
    
    \scalebox{0.78}{Symbols} &
    \scalebox{0.78}{32.66} &\scalebox{0.78}{12.51} &\scalebox{0.78}{32.60} &\scalebox{0.78}{17.78} &\scalebox{0.78}{23.89} &
    \scalebox{0.78}{86.83} &\scalebox{0.78}{89.20} &\scalebox{0.78}{86.50} &\scalebox{0.78}{86.40} &\scalebox{0.78}{87.23} &
    \scalebox{0.78}{86.43} &\scalebox{0.78}{88.34} &\scalebox{0.78}{86.03} &\scalebox{0.78}{86.02} &\scalebox{0.78}{86.70} &
    \scalebox{0.78}{88.64} &\scalebox{0.78}{90.96} &\scalebox{0.78}{88.29} &\scalebox{0.78}{88.59} &\scalebox{0.78}{89.12} \\
    
    \scalebox{0.78}{SyntheticControl} &
    \scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &
    \scalebox{0.78}{96.33} &\scalebox{0.78}{96.46} &\scalebox{0.78}{96.33} &\scalebox{0.78}{96.31} &\scalebox{0.78}{96.36} &
    \scalebox{0.78}{99.00} &\scalebox{0.78}{99.03} &\scalebox{0.78}{99.00} &\scalebox{0.78}{99.00} &\scalebox{0.78}{99.01} &
    \scalebox{0.78}{99.67} &\scalebox{0.78}{99.67} &\scalebox{0.78}{99.67} &\scalebox{0.78}{99.67} &\scalebox{0.78}{99.67} \\

    \scalebox{0.78}{ToeSegmentation1} &
    \scalebox{0.78}{53.51} &\scalebox{0.78}{64.06} &\scalebox{0.78}{50.97} &\scalebox{0.78}{37.27} &\scalebox{0.78}{51.45} &
    \scalebox{0.78}{65.79} &\scalebox{0.78}{65.70} &\scalebox{0.78}{65.51} &\scalebox{0.78}{65.52} &\scalebox{0.78}{65.63} &
    \scalebox{0.78}{85.53} &\scalebox{0.78}{85.69} &\scalebox{0.78}{85.32} &\scalebox{0.78}{85.43} &\scalebox{0.78}{85.49} &
    \scalebox{0.78}{71.49} &\scalebox{0.78}{71.97} &\scalebox{0.78}{70.97} &\scalebox{0.78}{70.95} &\scalebox{0.78}{71.34} \\

    \scalebox{0.78}{ToeSegmentation2} &
    \scalebox{0.78}{91.54} &\scalebox{0.78}{70.77} &\scalebox{0.78}{80.00} &\scalebox{0.78}{84.92} &\scalebox{0.78}{81.81} &
    \scalebox{0.78}{84.62} &\scalebox{0.78}{75.11} &\scalebox{0.78}{68.00} &\scalebox{0.78}{70.45} &\scalebox{0.78}{74.55} &
    \scalebox{0.78}{83.08} &\scalebox{0.78}{72.99} &\scalebox{0.78}{78.34} &\scalebox{0.78}{74.96} &\scalebox{0.78}{77.34} &
    \scalebox{0.78}{84.62} &\scalebox{0.78}{74.45} &\scalebox{0.78}{72.84} &\scalebox{0.78}{73.59} &\scalebox{0.78}{76.38} \\

    \scalebox{0.78}{Trace} &
    \scalebox{0.78}{81.00} &\scalebox{0.78}{77.50} &\scalebox{0.78}{75.42} &\scalebox{0.78}{70.87} &\scalebox{0.78}{76.20} &
    \scalebox{0.78}{84.00} &\scalebox{0.78}{87.47} &\scalebox{0.78}{85.78} &\scalebox{0.78}{83.04} &\scalebox{0.78}{85.07} &
    \scalebox{0.78}{75.00} &\scalebox{0.78}{85.80} &\scalebox{0.78}{77.68} &\scalebox{0.78}{69.92} &\scalebox{0.78}{77.10} &
    \scalebox{0.78}{92.00} &\scalebox{0.78}{91.62} &\scalebox{0.78}{92.10} &\scalebox{0.78}{91.69} &\scalebox{0.78}{91.85} \\

    \scalebox{0.78}{TwoPatterns} &
    \scalebox{0.78}{25.87} &\scalebox{0.78}{6.47} &\scalebox{0.78}{25.00} &\scalebox{0.78}{10.28} &\scalebox{0.78}{16.91} &
    \scalebox{0.78}{99.48} &\scalebox{0.78}{99.47} &\scalebox{0.78}{99.47} &\scalebox{0.78}{99.47} &\scalebox{0.78}{99.47} &
    \scalebox{0.78}{99.70} &\scalebox{0.78}{99.70} &\scalebox{0.78}{99.70} &\scalebox{0.78}{99.70} &\scalebox{0.78}{99.70} &
    \scalebox{0.78}{99.20} &\scalebox{0.78}{99.20} &\scalebox{0.78}{99.21} &\scalebox{0.78}{99.20} &\scalebox{0.78}{99.20} \\

    \scalebox{0.78}{UMD} &
    \scalebox{0.78}{99.31} &\scalebox{0.78}{99.32} &\scalebox{0.78}{99.31} &\scalebox{0.78}{99.31} &\scalebox{0.78}{99.31} &
    \scalebox{0.78}{98.65} &\scalebox{0.78}{98.65} &\scalebox{0.78}{98.65} &\scalebox{0.78}{98.65} &\scalebox{0.78}{98.65} &
    \scalebox{0.78}{97.92} &\scalebox{0.78}{97.99} &\scalebox{0.78}{97.92} &\scalebox{0.78}{97.90} &\scalebox{0.78}{97.93} &
    \scalebox{0.78}{92.50} &\scalebox{0.78}{92.12} &\scalebox{0.78}{92.60} &\scalebox{0.78}{92.19} &\scalebox{0.78}{92.35} \\

    \scalebox{0.78}{UWaveGestureLibraryX} &
    \scalebox{0.78}{12.62} &\scalebox{0.78}{1.58} &\scalebox{0.78}{12.50} &\scalebox{0.78}{2.80} &\scalebox{0.78}{7.38} &
    \scalebox{0.78}{78.34} &\scalebox{0.78}{76.55} &\scalebox{0.78}{78.04} &\scalebox{0.78}{76.65} &\scalebox{0.78}{77.39} &
    \scalebox{0.78}{80.43} &\scalebox{0.78}{79.23} &\scalebox{0.78}{80.21} &\scalebox{0.78}{79.59} &\scalebox{0.78}{79.87} &
    \scalebox{0.78}{71.55} &\scalebox{0.78}{69.61} &\scalebox{0.78}{71.29} &\scalebox{0.78}{70.12} &\scalebox{0.78}{70.64} \\

    \scalebox{0.78}{UWaveGestureLibraryY} &
    \scalebox{0.78}{79.65} &\scalebox{0.78}{79.44} &\scalebox{0.78}{79.75} &\scalebox{0.78}{79.24} &\scalebox{0.78}{79.52} &
    \scalebox{0.78}{67.00} &\scalebox{0.78}{66.65} &\scalebox{0.78}{67.07} &\scalebox{0.78}{66.19} &\scalebox{0.78}{66.73} &
    \scalebox{0.78}{70.94} &\scalebox{0.78}{70.43} &\scalebox{0.78}{71.02} &\scalebox{0.78}{70.42} &\scalebox{0.78}{70.70} &
    \scalebox{0.78}{63.51} &\scalebox{0.78}{62.81} &\scalebox{0.78}{63.61} &\scalebox{0.78}{62.82} &\scalebox{0.78}{63.19} \\

    \scalebox{0.78}{UWaveGestureLibraryZ} &
    \scalebox{0.78}{25.57} &\scalebox{0.78}{19.48} &\scalebox{0.78}{25.70} &\scalebox{0.78}{17.02} &\scalebox{0.78}{21.94} &
    \scalebox{0.78}{69.29} &\scalebox{0.78}{68.37} &\scalebox{0.78}{69.50} &\scalebox{0.78}{67.78} &\scalebox{0.78}{68.73} &
    \scalebox{0.78}{73.28} &\scalebox{0.78}{72.34} &\scalebox{0.78}{73.45} &\scalebox{0.78}{72.57} &\scalebox{0.78}{72.91} &
    \scalebox{0.78}{65.27} &\scalebox{0.78}{63.95} &\scalebox{0.78}{65.45} &\scalebox{0.78}{64.28} &\scalebox{0.78}{64.74} \\

    \scalebox{0.78}{Wafer} &
    \scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &
    \scalebox{0.78}{99.58} &\scalebox{0.78}{98.72} &\scalebox{0.78}{99.10} &\scalebox{0.78}{98.91} &\scalebox{0.78}{99.08} &
    \scalebox{0.78}{99.37} &\scalebox{0.78}{98.83} &\scalebox{0.78}{97.86} &\scalebox{0.78}{98.34} &\scalebox{0.78}{98.60} &
    \scalebox{0.78}{99.53} &\scalebox{0.78}{99.07} &\scalebox{0.78}{98.48} &\scalebox{0.78}{98.77} &\scalebox{0.78}{98.96} \\

    \scalebox{0.78}{WordSynonyms} &
    \scalebox{0.78}{56.74} &\scalebox{0.78}{46.59} &\scalebox{0.78}{39.49} &\scalebox{0.78}{39.50} &\scalebox{0.78}{45.58} &
    \scalebox{0.78}{58.15} &\scalebox{0.78}{47.43} &\scalebox{0.78}{40.03} &\scalebox{0.78}{40.83} &\scalebox{0.78}{46.61} &
    \scalebox{0.78}{61.76} &\scalebox{0.78}{54.59} &\scalebox{0.78}{45.32} &\scalebox{0.78}{46.33} &\scalebox{0.78}{52.00} &
    \scalebox{0.78}{56.74} &\scalebox{0.78}{43.82} &\scalebox{0.78}{38.11} &\scalebox{0.78}{37.75} &\scalebox{0.78}{44.11} \\

    \midrule
    
    \multicolumn{1}{c}{\scalebox{0.78}{{$1^{\text{st}}$ Count}}} & 
    \multicolumn{4}{c}{\textbf{\scalebox{0.78}{73}}} & 
    \multicolumn{2}{c}{\scalebox{0.78}{6}} & 
    \multicolumn{2}{c}{\scalebox{0.78}{2}} & 
    \multicolumn{2}{c}{\scalebox{0.78}{7}} & 
    \multicolumn{2}{c}{\scalebox{0.78}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.78}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.78}{0}} &  
    \multicolumn{2}{c}{\scalebox{0.78}{2}} & 
    \multicolumn{2}{c}{\scalebox{0.78}{0}} \\
    
    \midrule
    \midrule
  \end{tabular}
    \end{small}
  \end{threeparttable}
  }
\end{table*}

==> tables/classification_few_5.tex <==
\begin{table*}[htbp]
\caption{Classification-5 (few-shot)}\label{tab:classification_few_5}
\vskip 0.1in
\centering
\resizebox{1.75\columnwidth}{!}{
\begin{threeparttable}
\begin{small}
\renewcommand{\multirowsetup}{\centering}
\setlength{\tabcolsep}{7pt}
\begin{tabular}{c|c|c|cccc|c}
\toprule
\hline

\multicolumn{2}{c}{Scenarios} & Models & Accuracy (\%) & Precision (\%) & Recall (\%) & F1 (\%) & Avg (\%) \\


\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{16}{*}[-3ex]{\rotatebox{90}{\shortstack{DistalPhalanxTW \\ $\downarrow$ \\ ProximalPhalanxOutlineCorrect}}}

& \multirow{4}{*}[0ex]{\shortstack{Full Data}}
& MICN & 84.88 & 85.82 & \textbf{78.42} & \textbf{80.73} & 82.46 \\
& & TimesNet & \textbf{85.22} & \textbf{88.80} & 77.51 & 80.43 & \textbf{82.99} \\
& & PatchTST & 78.69 & 75.80 & 73.03 & 74.06 & 75.39 \\
& & OneFitsAll & 79.73 & 76.00 & 76.12 & 76.35 & 77.20 \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (10\%)}}
& Random init. & 75.26 & 71.93 & 67.01 & 68.21 & 70.60 \\
\cmidrule(lr){3-8}
& & MICN & 80.38 & 79.46 & 78.00 & 78.67 & 79.13 \\
& & TimesNet & 77.32 & 73.77 & 73.19 & 73.46 & 74.44 \\
& & PatchTST & 78.69 & 81.61 & 68.06 & 69.95 & 74.57 \\
& & OneFitsAll & 77.66 & 74.35 & 72.27 & 73.09 & 74.34 \\
& & \myformer & \textbf{86.25} & \textbf{84.11} & \textbf{84.11} & \textbf{84.11} & \textbf{84.65} \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (5\%)}}
& Random init. & 68.38 & 34.19 & 50.00 & 40.61 & 48.30 \\
\cmidrule(lr){3-8}
& & MICN & 81.79 & 80.32 & 75.87 & 77.42 & 78.85 \\
& & TimesNet & 78.01 & 78.99 & 67.85 & 69.60 & 73.61 \\
& & PatchTST & 78.35 & 76.20 & 71.02 & 72.52 & 74.52 \\
& & OneFitsAll & 76.98 & 74.22 & 69.43 & 70.78 & 72.85 \\
& & \myformer & \textbf{84.54} & \textbf{87.68} & \textbf{76.71} & \textbf{79.52} & \textbf{82.11} \\



\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{16}{*}[-3ex]{\rotatebox{90}{\shortstack{- \\ $\downarrow$ \\ -}}}

& \multirow{4}{*}[0ex]{\shortstack{Full Data}}
& MICN & - & - & - & - & - \\
& & TimesNet & - & - & - & - & - \\
& & PatchTST & - & - & - & - & - \\
& & OneFitsAll & - & - & - & - & - \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (10\%)}}
& Random init. & - & - & - & - & - \\
\cmidrule(lr){3-8}
& & MICN & - & - & - & - & - \\
& & TimesNet & - & - & - & - & - \\
& & PatchTST & - & - & - & - & - \\
& & OneFitsAll & - & - & - & - & - \\
& & \myformer & - & - & - & - & - \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (5\%)}}
& Random init. & - & - & - & - & - \\
\cmidrule(lr){3-8}
& & MICN & - & - & - & - & - \\
& & TimesNet & - & - & - & - & - \\
& & PatchTST & - & - & - & - & - \\
& & OneFitsAll & - & - & - & - & - \\
& & \myformer & - & - & - & - & - \\


\hline
\bottomrule
\end{tabular}
\end{small}
\end{threeparttable}
}
\end{table*}

==> tables/forecasting.tex <==
\begin{table*}[htbp]
  \caption{CWT-adapter in Forecasting (cross-zero) Task. \\ Forecasting2Forecasting}\label{tab:forecasting}
  \vskip 0.05in
  \centering
  \resizebox{2\columnwidth}{!}{
  \begin{threeparttable}
  \begin{small}
  \renewcommand{\multirowsetup}{\centering}
  \setlength{\tabcolsep}{0.8pt}
  \begin{tabular}{c|c|cc|cc|cc||cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}

    \hline
    \hline
    \multicolumn{2}{c}{\multirow{1}{*}{Source}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Scratch-1.0}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Scratch-0.1}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Scratch-0.05}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{ETTm1}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{ETTm2}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{ETTh1}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{ETTh2}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Exchange}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Weather}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Sunspot}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{RiverFlow}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{SolarPower}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{WindPower}}} \\
    
    \hline
    
    \multicolumn{2}{c}{\scalebox{0.76}{MaskRatio}} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} \\
    
    \hline
    
    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ETTm1}}}

    & \scalebox{0.78}{96} &
    \scalebox{0.78}{0.360} & \scalebox{0.78}{0.380} &
    \scalebox{0.78}{0.383} & \scalebox{0.78}{0.395} &
    \scalebox{0.78}{0.504} & \scalebox{0.78}{0.461} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.500} & \scalebox{0.78}{0.447} &
    \scalebox{0.78}{0.747} & \scalebox{0.78}{0.552} &
    \scalebox{0.78}{0.833} & \scalebox{0.78}{0.573} &
    \scalebox{0.78}{1.435} & \scalebox{0.78}{0.727} &
    \scalebox{0.78}{1.144} & \scalebox{0.78}{0.673} &
    \scalebox{0.78}{0.750} & \scalebox{0.78}{0.561} &
    \scalebox{0.78}{0.851} & \scalebox{0.78}{0.593} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{192} &
    \scalebox{0.78}{0.397} & \scalebox{0.78}{0.397} &
    \scalebox{0.78}{0.414} & \scalebox{0.78}{0.409} &
    \scalebox{0.78}{0.504} & \scalebox{0.78}{0.461} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.515} & \scalebox{0.78}{0.457} &
    \scalebox{0.78}{0.781} & \scalebox{0.78}{0.571} &
    \scalebox{0.78}{0.840} & \scalebox{0.78}{0.586} &
    \scalebox{0.78}{1.400} & \scalebox{0.78}{0.731} &
    \scalebox{0.78}{1.107} & \scalebox{0.78}{0.671} &
    \scalebox{0.78}{0.744} & \scalebox{0.78}{0.566} &
    \scalebox{0.78}{0.916} & \scalebox{0.78}{0.647} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{336} &
    \scalebox{0.78}{0.428} & \scalebox{0.78}{0.417} &
    \scalebox{0.78}{0.446} & \scalebox{0.78}{0.430} &
    \scalebox{0.78}{0.459} & \scalebox{0.78}{0.438} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.542} & \scalebox{0.78}{0.474} &
    \scalebox{0.78}{0.773} & \scalebox{0.78}{0.575} &
    \scalebox{0.78}{0.842} & \scalebox{0.78}{0.593} &
    \scalebox{0.78}{1.440} & \scalebox{0.78}{0.753} &
    \scalebox{0.78}{0.949} & \scalebox{0.78}{0.621} &
    \scalebox{0.78}{0.786} & \scalebox{0.78}{0.586} &
    \scalebox{0.78}{0.909} & \scalebox{0.78}{0.643} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{720} &
    \scalebox{0.78}{0.469} & \scalebox{0.78}{0.447} &
    \scalebox{0.78}{0.504} & \scalebox{0.78}{0.461} &
    \scalebox{0.78}{0.522} & \scalebox{0.78}{0.472} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.581} & \scalebox{0.78}{0.499} &
    \scalebox{0.78}{0.828} & \scalebox{0.78}{0.583} &
    \scalebox{0.78}{0.851} & \scalebox{0.78}{0.610} &
    \scalebox{0.78}{1.313} & \scalebox{0.78}{0.730} &
    \scalebox{0.78}{0.974} & \scalebox{0.78}{0.643} &
    \scalebox{0.78}{0.853} & \scalebox{0.78}{0.619} &
    \scalebox{0.78}{0.953} & \scalebox{0.78}{0.665} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \cline{2-28}

    & \scalebox{0.78}{Avg} &
    \scalebox{0.78}{0.413} & \scalebox{0.78}{0.413} &
    \scalebox{0.78}{0.437} & \scalebox{0.78}{0.437} &
    \scalebox{0.78}{0.497} & \scalebox{0.78}{0.497} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.534} & \scalebox{0.78}{0.534} &
    \scalebox{0.78}{0.782} & \scalebox{0.78}{0.782} &
    \scalebox{0.78}{0.842} & \scalebox{0.78}{0.842} &
    \scalebox{0.78}{1.397} & \scalebox{0.78}{1.397} &
    \scalebox{0.78}{1.043} & \scalebox{0.78}{1.043} &
    \scalebox{0.78}{0.783} & \scalebox{0.78}{0.783} &
    \scalebox{0.78}{0.907} & \scalebox{0.78}{0.907} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \hline

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ETTm2}}}

    & \scalebox{0.78}{96} &
    \scalebox{0.78}{0.183} & \scalebox{0.78}{0.266} &
    \scalebox{0.78}{0.189} & \scalebox{0.78}{0.273} &
    \scalebox{0.78}{0.194} & \scalebox{0.78}{0.278} &
    \scalebox{0.78}{0.191} & \scalebox{0.78}{0.263} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.214} & \scalebox{0.78}{0.299} &
    \scalebox{0.78}{0.215} & \scalebox{0.78}{0.301} &
    \scalebox{0.78}{0.270} & \scalebox{0.78}{0.342} &
    \scalebox{0.78}{0.277} & \scalebox{0.78}{0.345} &
    \scalebox{0.78}{0.216} & \scalebox{0.78}{0.299} &
    \scalebox{0.78}{0.219} & \scalebox{0.78}{0.298} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{192} &
    \scalebox{0.78}{0.247} & \scalebox{0.78}{0.305} &
    \scalebox{0.78}{0.251} & \scalebox{0.78}{0.310} &
    \scalebox{0.78}{0.254} & \scalebox{0.78}{0.312} &
    \scalebox{0.78}{0.254} & \scalebox{0.78}{0.303} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.278} & \scalebox{0.78}{0.338} &
    \scalebox{0.78}{0.280} & \scalebox{0.78}{0.341} &
    \scalebox{0.78}{0.334} & \scalebox{0.78}{0.377} &
    \scalebox{0.78}{0.319} & \scalebox{0.78}{0.368} &
    \scalebox{0.78}{0.273} & \scalebox{0.78}{0.331} &
    \scalebox{0.78}{0.305} & \scalebox{0.78}{0.352} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{336} &
    \scalebox{0.78}{0.308} & \scalebox{0.78}{0.343} &
    \scalebox{0.78}{0.311} & \scalebox{0.78}{0.347} &
    \scalebox{0.78}{0.314} & \scalebox{0.78}{0.349} &
    \scalebox{0.78}{0.312} & \scalebox{0.78}{0.340} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.331} & \scalebox{0.78}{0.368} &
    \scalebox{0.78}{0.338} & \scalebox{0.78}{0.376} &
    \scalebox{0.78}{0.402} & \scalebox{0.78}{0.415} &
    \scalebox{0.78}{0.357} & \scalebox{0.78}{0.384} &
    \scalebox{0.78}{0.334} & \scalebox{0.78}{0.367} &
    \scalebox{0.78}{0.360} & \scalebox{0.78}{0.384} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{720} &
    \scalebox{0.78}{0.408} & \scalebox{0.78}{0.399} &
    \scalebox{0.78}{0.411} & \scalebox{0.78}{0.401} &
    \scalebox{0.78}{0.413} & \scalebox{0.78}{0.403} &
    \scalebox{0.78}{0.413} & \scalebox{0.78}{0.399} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.439} & \scalebox{0.78}{0.430} &
    \scalebox{0.78}{0.432} & \scalebox{0.78}{0.422} &
    \scalebox{0.78}{0.499} & \scalebox{0.78}{0.460} &
    \scalebox{0.78}{0.457} & \scalebox{0.78}{0.436} &
    \scalebox{0.78}{0.439} & \scalebox{0.78}{0.422} &
    \scalebox{0.78}{0.459} & \scalebox{0.78}{0.436} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \cline{2-28}

    & \scalebox{0.78}{Avg} &
    \scalebox{0.78}{0.286} & \scalebox{0.78}{0.286} &
    \scalebox{0.78}{0.290} & \scalebox{0.78}{0.290} &
    \scalebox{0.78}{0.294} & \scalebox{0.78}{0.294} &
    \scalebox{0.78}{0.292} & \scalebox{0.78}{0.292} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.316} & \scalebox{0.78}{0.316} &
    \scalebox{0.78}{0.316} & \scalebox{0.78}{0.316} &
    \scalebox{0.78}{0.376} & \scalebox{0.78}{0.376} &
    \scalebox{0.78}{0.353} & \scalebox{0.78}{0.353} &
    \scalebox{0.78}{0.316} & \scalebox{0.78}{0.316} &
    \scalebox{0.78}{0.336} & \scalebox{0.78}{0.336} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \hline

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ETTh1}}}

    & \scalebox{0.78}{96} &
    \scalebox{0.78}{0.403} & \scalebox{0.78}{0.413} &
    \scalebox{0.78}{0.513} & \scalebox{0.78}{0.475} &
    \scalebox{0.78}{0.585} & \scalebox{0.78}{0.506} &
    \scalebox{0.78}{0.671} & \scalebox{0.78}{0.542} &
    \scalebox{0.78}{0.703} & \scalebox{0.78}{0.552} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.527} & \scalebox{0.78}{0.480} &
    \scalebox{0.78}{0.809} & \scalebox{0.78}{0.598} &
    \scalebox{0.78}{0.794} & \scalebox{0.78}{0.587} &
    \scalebox{0.78}{0.698} & \scalebox{0.78}{0.556} &
    \scalebox{0.78}{0.799} & \scalebox{0.78}{0.613} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{192} &
    \scalebox{0.78}{0.454} & \scalebox{0.78}{0.445} &
    \scalebox{0.78}{0.499} & \scalebox{0.78}{0.469} &
    \scalebox{0.78}{0.606} & \scalebox{0.78}{0.520} &
    \scalebox{0.78}{0.659} & \scalebox{0.78}{0.543} &
    \scalebox{0.78}{0.695} & \scalebox{0.78}{0.553} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.587} & \scalebox{0.78}{0.521} &
    \scalebox{0.78}{0.810} & \scalebox{0.78}{0.602} &
    \scalebox{0.78}{0.795} & \scalebox{0.78}{0.595} &
    \scalebox{0.78}{0.695} & \scalebox{0.78}{0.563} &
    \scalebox{0.78}{0.911} & \scalebox{0.78}{0.675} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{336} &
    \scalebox{0.78}{0.487} & \scalebox{0.78}{0.462} &
    \scalebox{0.78}{0.525} & \scalebox{0.78}{0.480} &
    \scalebox{0.78}{0.595} & \scalebox{0.78}{0.520} &
    \scalebox{0.78}{0.671} & \scalebox{0.78}{0.554} &
    \scalebox{0.78}{0.707} & \scalebox{0.78}{0.564} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{1.084} & \scalebox{0.78}{0.702} &
    \scalebox{0.78}{0.819} & \scalebox{0.78}{0.613} &
    \scalebox{0.78}{0.791} & \scalebox{0.78}{0.604} &
    \scalebox{0.78}{0.717} & \scalebox{0.78}{0.582} &
    \scalebox{0.78}{0.903} & \scalebox{0.78}{0.674} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{720} &
    \scalebox{0.78}{0.549} & \scalebox{0.78}{0.502} &
    \scalebox{0.78}{0.531} & \scalebox{0.78}{0.502} &
    \scalebox{0.78}{0.609} & \scalebox{0.78}{0.551} &
    \scalebox{0.78}{0.660} & \scalebox{0.78}{0.569} &
    \scalebox{0.78}{0.675} & \scalebox{0.78}{0.573} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.652} & \scalebox{0.78}{0.572} &
    \scalebox{0.78}{0.805} & \scalebox{0.78}{0.623} &
    \scalebox{0.78}{0.767} & \scalebox{0.78}{0.614} &
    \scalebox{0.78}{0.743} & \scalebox{0.78}{0.613} &
    \scalebox{0.78}{0.917} & \scalebox{0.78}{0.691} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \cline{2-28}

    & \scalebox{0.78}{Avg} &
    \scalebox{0.78}{0.473} & \scalebox{0.78}{0.473} &
    \scalebox{0.78}{0.517} & \scalebox{0.78}{0.517} &
    \scalebox{0.78}{0.599} & \scalebox{0.78}{0.599} &
    \scalebox{0.78}{0.665} & \scalebox{0.78}{0.665} &
    \scalebox{0.78}{0.695} & \scalebox{0.78}{0.695} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.713} & \scalebox{0.78}{0.713} &
    \scalebox{0.78}{0.811} & \scalebox{0.78}{0.811} &
    \scalebox{0.78}{0.787} & \scalebox{0.78}{0.787} &
    \scalebox{0.78}{0.713} & \scalebox{0.78}{0.713} &
    \scalebox{0.78}{0.883} & \scalebox{0.78}{0.883} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \hline

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ETTh2}}}

    & \scalebox{0.78}{96} &
    \scalebox{0.78}{0.298} & \scalebox{0.78}{0.346} &
    \scalebox{0.78}{0.328} & \scalebox{0.78}{0.370} &
    \scalebox{0.78}{0.341} & \scalebox{0.78}{0.379} &
    \scalebox{0.78}{0.344} & \scalebox{0.78}{0.380} &
    \scalebox{0.78}{0.326} & \scalebox{0.78}{0.370} &
    \scalebox{0.78}{0.297} & \scalebox{0.78}{0.343} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.374} & \scalebox{0.78}{0.389} &
    \scalebox{0.78}{0.362} & \scalebox{0.78}{0.389} &
    \scalebox{0.78}{0.327} & \scalebox{0.78}{0.371} &
    \scalebox{0.78}{0.351} & \scalebox{0.78}{0.385} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{192} &
    \scalebox{0.78}{0.378} & \scalebox{0.78}{0.403} &
    \scalebox{0.78}{0.406} & \scalebox{0.78}{0.415} &
    \scalebox{0.78}{0.420} & \scalebox{0.78}{0.424} &
    \scalebox{0.78}{0.430} & \scalebox{0.78}{0.424} &
    \scalebox{0.78}{0.411} & \scalebox{0.78}{0.415} &
    \scalebox{0.78}{0.395} & \scalebox{0.78}{0.403} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.456} & \scalebox{0.78}{0.433} &
    \scalebox{0.78}{0.426} & \scalebox{0.78}{0.425} &
    \scalebox{0.78}{0.405} & \scalebox{0.78}{0.414} &
    \scalebox{0.78}{0.459} & \scalebox{0.78}{0.451} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{336} &
    \scalebox{0.78}{0.414} & \scalebox{0.78}{0.439} &
    \scalebox{0.78}{0.436} & \scalebox{0.78}{0.443} &
    \scalebox{0.78}{0.449} & \scalebox{0.78}{0.450} &
    \scalebox{0.78}{0.460} & \scalebox{0.78}{0.452} &
    \scalebox{0.78}{0.450} & \scalebox{0.78}{0.448} &
    \scalebox{0.78}{0.418} & \scalebox{0.78}{0.429} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.511} & \scalebox{0.78}{0.472} &
    \scalebox{0.78}{0.459} & \scalebox{0.78}{0.456} &
    \scalebox{0.78}{0.451} & \scalebox{0.78}{0.449} &
    \scalebox{0.78}{0.481} & \scalebox{0.78}{0.474} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{720} &
    \scalebox{0.78}{0.423} & \scalebox{0.78}{0.443} &
    \scalebox{0.78}{0.451} & \scalebox{0.78}{0.460} &
    \scalebox{0.78}{0.448} & \scalebox{0.78}{0.459} &
    \scalebox{0.78}{0.487} & \scalebox{0.78}{0.477} &
    \scalebox{0.78}{0.446} & \scalebox{0.78}{0.455} &
    \scalebox{0.78}{0.428} & \scalebox{0.78}{0.446} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.512} & \scalebox{0.78}{0.482} &
    \scalebox{0.78}{0.462} & \scalebox{0.78}{0.465} &
    \scalebox{0.78}{0.455} & \scalebox{0.78}{0.459} &
    \scalebox{0.78}{0.485} & \scalebox{0.78}{0.481} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \cline{2-28}

    & \scalebox{0.78}{Avg} &
    \scalebox{0.78}{0.378} & \scalebox{0.78}{0.378} &
    \scalebox{0.78}{0.405} & \scalebox{0.78}{0.405} &
    \scalebox{0.78}{0.414} & \scalebox{0.78}{0.414} &
    \scalebox{0.78}{0.430} & \scalebox{0.78}{0.430} &
    \scalebox{0.78}{0.408} & \scalebox{0.78}{0.408} &
    \scalebox{0.78}{0.384} & \scalebox{0.78}{0.384} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.463} & \scalebox{0.78}{0.463} &
    \scalebox{0.78}{0.427} & \scalebox{0.78}{0.427} &
    \scalebox{0.78}{0.410} & \scalebox{0.78}{0.410} &
    \scalebox{0.78}{0.444} & \scalebox{0.78}{0.444} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \hline

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{Exchange}}}

    & \scalebox{0.78}{96} &
    \scalebox{0.78}{0.084} & \scalebox{0.78}{0.203} &
    \scalebox{0.78}{0.103} & \scalebox{0.78}{0.227} &
    \scalebox{0.78}{0.109} & \scalebox{0.78}{0.235} &
    \scalebox{0.78}{0.117} & \scalebox{0.78}{0.253} &
    \scalebox{0.78}{0.095} & \scalebox{0.78}{0.223} &
    \scalebox{0.78}{0.112} & \scalebox{0.78}{0.237} &
    \scalebox{0.78}{0.106} & \scalebox{0.78}{0.229} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.136} & \scalebox{0.78}{0.267} &
    \scalebox{0.78}{0.109} & \scalebox{0.78}{0.242} &
    \scalebox{0.78}{0.090} & \scalebox{0.78}{0.220} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{192} &
    \scalebox{0.78}{0.175} & \scalebox{0.78}{0.298} &
    \scalebox{0.78}{0.199} & \scalebox{0.78}{0.319} &
    \scalebox{0.78}{0.221} & \scalebox{0.78}{0.340} &
    \scalebox{0.78}{0.219} & \scalebox{0.78}{0.350} &
    \scalebox{0.78}{0.195} & \scalebox{0.78}{0.324} &
    \scalebox{0.78}{0.208} & \scalebox{0.78}{0.326} &
    \scalebox{0.78}{0.211} & \scalebox{0.78}{0.330} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.214} & \scalebox{0.78}{0.344} &
    \scalebox{0.78}{0.206} & \scalebox{0.78}{0.337} &
    \scalebox{0.78}{0.198} & \scalebox{0.78}{0.331} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{336} &
    \scalebox{0.78}{0.322} & \scalebox{0.78}{0.410} &
    \scalebox{0.78}{0.351} & \scalebox{0.78}{0.431} &
    \scalebox{0.78}{0.370} & \scalebox{0.78}{0.445} &
    \scalebox{0.78}{0.394} & \scalebox{0.78}{0.471} &
    \scalebox{0.78}{0.379} & \scalebox{0.78}{0.457} &
    \scalebox{0.78}{0.359} & \scalebox{0.78}{0.435} &
    \scalebox{0.78}{0.356} & \scalebox{0.78}{0.435} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.385} & \scalebox{0.78}{0.464} &
    \scalebox{0.78}{0.365} & \scalebox{0.78}{0.450} &
    \scalebox{0.78}{0.375} & \scalebox{0.78}{0.453} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{720} &
    \scalebox{0.78}{1.008} & \scalebox{0.78}{0.803} &
    \scalebox{0.78}{1.076} & \scalebox{0.78}{0.842} &
    \scalebox{0.78}{1.113} & \scalebox{0.78}{0.860} &
    \scalebox{0.78}{1.087} & \scalebox{0.78}{0.847} &
    \scalebox{0.78}{1.075} & \scalebox{0.78}{0.840} &
    \scalebox{0.78}{0.956} & \scalebox{0.78}{0.743} &
    \scalebox{0.78}{0.879} & \scalebox{0.78}{0.711} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{1.082} & \scalebox{0.78}{0.846} &
    \scalebox{0.78}{1.015} & \scalebox{0.78}{0.815} &
    \scalebox{0.78}{1.024} & \scalebox{0.78}{0.819} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \cline{2-28}

    & \scalebox{0.78}{Avg} &
    \scalebox{0.78}{0.397} & \scalebox{0.78}{0.397} &
    \scalebox{0.78}{0.432} & \scalebox{0.78}{0.432} &
    \scalebox{0.78}{0.453} & \scalebox{0.78}{0.453} &
    \scalebox{0.78}{0.454} & \scalebox{0.78}{0.454} &
    \scalebox{0.78}{0.436} & \scalebox{0.78}{0.436} &
    \scalebox{0.78}{0.409} & \scalebox{0.78}{0.409} &
    \scalebox{0.78}{0.388} & \scalebox{0.78}{0.388} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.454} & \scalebox{0.78}{0.454} &
    \scalebox{0.78}{0.424} & \scalebox{0.78}{0.424} &
    \scalebox{0.78}{0.422} & \scalebox{0.78}{0.422} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \hline

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{Weather}}}

    & \scalebox{0.78}{96} &
    \scalebox{0.78}{0.183} & \scalebox{0.78}{0.220} &
    \scalebox{0.78}{0.196} & \scalebox{0.78}{0.237} &
    \scalebox{0.78}{0.183} & \scalebox{0.78}{0.224} &
    \scalebox{0.78}{0.210} & \scalebox{0.78}{0.254} &
    \scalebox{0.78}{0.202} & \scalebox{0.78}{0.247} &
    \scalebox{0.78}{0.202} & \scalebox{0.78}{0.254} &
    \scalebox{0.78}{0.197} & \scalebox{0.78}{0.246} &
    \scalebox{0.78}{0.252} & \scalebox{0.78}{0.272} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.181} & \scalebox{0.78}{0.235} &
    \scalebox{0.78}{0.186} & \scalebox{0.78}{0.227} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{192} &
    \scalebox{0.78}{0.222} & \scalebox{0.78}{0.252} &
    \scalebox{0.78}{0.241} & \scalebox{0.78}{0.273} &
    \scalebox{0.78}{0.224} & \scalebox{0.78}{0.256} &
    \scalebox{0.78}{0.261} & \scalebox{0.78}{0.291} &
    \scalebox{0.78}{0.245} & \scalebox{0.78}{0.279} &
    \scalebox{0.78}{0.253} & \scalebox{0.78}{0.292} &
    \scalebox{0.78}{0.263} & \scalebox{0.78}{0.296} &
    \scalebox{0.78}{0.293} & \scalebox{0.78}{0.304} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.226} & \scalebox{0.78}{0.269} &
    \scalebox{0.78}{0.238} & \scalebox{0.78}{0.266} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{336} &
    \scalebox{0.78}{0.267} & \scalebox{0.78}{0.285} &
    \scalebox{0.78}{0.269} & \scalebox{0.78}{0.287} &
    \scalebox{0.78}{0.269} & \scalebox{0.78}{0.288} &
    \scalebox{0.78}{0.298} & \scalebox{0.78}{0.313} &
    \scalebox{0.78}{0.285} & \scalebox{0.78}{0.307} &
    \scalebox{0.78}{0.302} & \scalebox{0.78}{0.325} &
    \scalebox{0.78}{0.330} & \scalebox{0.78}{0.337} &
    \scalebox{0.78}{0.353} & \scalebox{0.78}{0.346} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.275} & \scalebox{0.78}{0.301} &
    \scalebox{0.78}{0.288} & \scalebox{0.78}{0.305} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{720} &
    \scalebox{0.78}{0.322} & \scalebox{0.78}{0.323} &
    \scalebox{0.78}{0.323} & \scalebox{0.78}{0.324} &
    \scalebox{0.78}{0.324} & \scalebox{0.78}{0.326} &
    \scalebox{0.78}{0.364} & \scalebox{0.78}{0.357} &
    \scalebox{0.78}{0.340} & \scalebox{0.78}{0.344} &
    \scalebox{0.78}{0.403} & \scalebox{0.78}{0.392} &
    \scalebox{0.78}{0.373} & \scalebox{0.78}{0.368} &
    \scalebox{0.78}{0.386} & \scalebox{0.78}{0.364} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.336} & \scalebox{0.78}{0.341} &
    \scalebox{0.78}{0.340} & \scalebox{0.78}{0.339} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \cline{2-28}

    & \scalebox{0.78}{Avg} &
    \scalebox{0.78}{0.248} & \scalebox{0.78}{0.248} &
    \scalebox{0.78}{0.257} & \scalebox{0.78}{0.257} &
    \scalebox{0.78}{0.250} & \scalebox{0.78}{0.250} &
    \scalebox{0.78}{0.283} & \scalebox{0.78}{0.283} &
    \scalebox{0.78}{0.268} & \scalebox{0.78}{0.268} &
    \scalebox{0.78}{0.290} & \scalebox{0.78}{0.290} &
    \scalebox{0.78}{0.291} & \scalebox{0.78}{0.291} &
    \scalebox{0.78}{0.321} & \scalebox{0.78}{0.321} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.255} & \scalebox{0.78}{0.255} &
    \scalebox{0.78}{0.263} & \scalebox{0.78}{0.263} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \hline

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{Sunspot}}}

    & \scalebox{0.78}{96} &
    \scalebox{0.78}{0.318} & \scalebox{0.78}{0.399} &
    \scalebox{0.78}{0.322} & \scalebox{0.78}{0.403} &
    \scalebox{0.78}{0.324} & \scalebox{0.78}{0.405} &
    \scalebox{0.78}{0.424} & \scalebox{0.78}{0.457} &
    \scalebox{0.78}{0.412} & \scalebox{0.78}{0.452} &
    \scalebox{0.78}{0.392} & \scalebox{0.78}{0.443} &
    \scalebox{0.78}{0.387} & \scalebox{0.78}{0.441} &
    \scalebox{0.78}{0.433} & \scalebox{0.78}{0.462} &
    \scalebox{0.78}{0.371} & \scalebox{0.78}{0.434} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.361} & \scalebox{0.78}{0.416} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{192} &
    \scalebox{0.78}{0.358} & \scalebox{0.78}{0.427} &
    \scalebox{0.78}{0.360} & \scalebox{0.78}{0.429} &
    \scalebox{0.78}{0.362} & \scalebox{0.78}{0.431} &
    \scalebox{0.78}{0.447} & \scalebox{0.78}{0.476} &
    \scalebox{0.78}{0.435} & \scalebox{0.78}{0.470} &
    \scalebox{0.78}{0.408} & \scalebox{0.78}{0.457} &
    \scalebox{0.78}{0.400} & \scalebox{0.78}{0.451} &
    \scalebox{0.78}{0.455} & \scalebox{0.78}{0.480} &
    \scalebox{0.78}{0.398} & \scalebox{0.78}{0.452} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.407} & \scalebox{0.78}{0.442} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{336} &
    \scalebox{0.78}{0.421} & \scalebox{0.78}{0.467} &
    \scalebox{0.78}{0.425} & \scalebox{0.78}{0.470} &
    \scalebox{0.78}{0.427} & \scalebox{0.78}{0.472} &
    \scalebox{0.78}{0.505} & \scalebox{0.78}{0.512} &
    \scalebox{0.78}{0.487} & \scalebox{0.78}{0.506} &
    \scalebox{0.78}{0.464} & \scalebox{0.78}{0.492} &
    \scalebox{0.78}{0.467} & \scalebox{0.78}{0.492} &
    \scalebox{0.78}{0.519} & \scalebox{0.78}{0.518} &
    \scalebox{0.78}{0.458} & \scalebox{0.78}{0.490} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.467} & \scalebox{0.78}{0.482} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{720} &
    \scalebox{0.78}{0.663} & \scalebox{0.78}{0.594} &
    \scalebox{0.78}{0.665} & \scalebox{0.78}{0.596} &
    \scalebox{0.78}{0.665} & \scalebox{0.78}{0.595} &
    \scalebox{0.78}{0.869} & \scalebox{0.78}{0.701} &
    \scalebox{0.78}{0.740} & \scalebox{0.78}{0.638} &
    \scalebox{0.78}{0.745} & \scalebox{0.78}{0.641} &
    \scalebox{0.78}{0.699} & \scalebox{0.78}{0.614} &
    \scalebox{0.78}{0.765} & \scalebox{0.78}{0.643} &
    \scalebox{0.78}{0.724} & \scalebox{0.78}{0.629} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.697} & \scalebox{0.78}{0.601} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \cline{2-28}

    & \scalebox{0.78}{Avg} &
    \scalebox{0.78}{0.440} & \scalebox{0.78}{0.440} &
    \scalebox{0.78}{0.443} & \scalebox{0.78}{0.443} &
    \scalebox{0.78}{0.445} & \scalebox{0.78}{0.445} &
    \scalebox{0.78}{0.561} & \scalebox{0.78}{0.561} &
    \scalebox{0.78}{0.518} & \scalebox{0.78}{0.518} &
    \scalebox{0.78}{0.502} & \scalebox{0.78}{0.502} &
    \scalebox{0.78}{0.488} & \scalebox{0.78}{0.488} &
    \scalebox{0.78}{0.543} & \scalebox{0.78}{0.543} &
    \scalebox{0.78}{0.488} & \scalebox{0.78}{0.488} &
     \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{0.483} & \scalebox{0.78}{0.483} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \hline

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{RiverFlow}}}

    & \scalebox{0.78}{96} &
    \scalebox{0.78}{1.158} & \scalebox{0.78}{0.527} &
    \scalebox{0.78}{1.171} & \scalebox{0.78}{0.536} &
    \scalebox{0.78}{1.192} & \scalebox{0.78}{0.545} &
    \scalebox{0.78}{1.527} & \scalebox{0.78}{0.717} &
    \scalebox{0.78}{1.536} & \scalebox{0.78}{0.724} &
    \scalebox{0.78}{1.410} & \scalebox{0.78}{0.698} &
    \scalebox{0.78}{1.424} & \scalebox{0.78}{0.705} &
    \scalebox{0.78}{1.786} & \scalebox{0.78}{0.728} &
    \scalebox{0.78}{1.465} & \scalebox{0.78}{0.698} &
    \scalebox{0.78}{1.327} & \scalebox{0.78}{0.679} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{192} &
    \scalebox{0.78}{1.289} & \scalebox{0.78}{0.566} &
    \scalebox{0.78}{1.297} & \scalebox{0.78}{0.578} &
    \scalebox{0.78}{1.299} & \scalebox{0.78}{0.576} &
    \scalebox{0.78}{1.678} & \scalebox{0.78}{0.766} &
    \scalebox{0.78}{1.694} & \scalebox{0.78}{0.786} &
    \scalebox{0.78}{1.521} & \scalebox{0.78}{0.734} &
    \scalebox{0.78}{1.519} & \scalebox{0.78}{0.739} &
    \scalebox{0.78}{1.987} & \scalebox{0.78}{0.798} &
    \scalebox{0.78}{1.563} & \scalebox{0.78}{0.733} &
    \scalebox{0.78}{1.442} & \scalebox{0.78}{0.717} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{336} &
    \scalebox{0.78}{1.198} & \scalebox{0.78}{0.551} &
    \scalebox{0.78}{1.199} & \scalebox{0.78}{0.565} &
    \scalebox{0.78}{1.209} & \scalebox{0.78}{0.561} &
    \scalebox{0.78}{1.557} & \scalebox{0.78}{0.719} &
    \scalebox{0.78}{1.537} & \scalebox{0.78}{0.737} &
    \scalebox{0.78}{1.387} & \scalebox{0.78}{0.686} &
    \scalebox{0.78}{1.452} & \scalebox{0.78}{0.718} &
    \scalebox{0.78}{1.906} & \scalebox{0.78}{0.791} &
    \scalebox{0.78}{1.508} & \scalebox{0.78}{0.709} &
    \scalebox{0.78}{1.377} & \scalebox{0.78}{0.680} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{720} &
    \scalebox{0.78}{1.182} & \scalebox{0.78}{0.543} &
    \scalebox{0.78}{1.190} & \scalebox{0.78}{0.551} &
    \scalebox{0.78}{1.191} & \scalebox{0.78}{0.552} &
    \scalebox{0.78}{1.937} & \scalebox{0.78}{0.884} &
    \scalebox{0.78}{1.477} & \scalebox{0.78}{0.715} &
    \scalebox{0.78}{1.534} & \scalebox{0.78}{0.778} &
    \scalebox{0.78}{1.360} & \scalebox{0.78}{0.671} &
    \scalebox{0.78}{1.880} & \scalebox{0.78}{0.786} &
    \scalebox{0.78}{1.446} & \scalebox{0.78}{0.691} &
    \scalebox{0.78}{1.384} & \scalebox{0.78}{0.671} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \cline{2-28}

    & \scalebox{0.78}{Avg} &
    \scalebox{0.78}{1.207} & \scalebox{0.78}{1.207} &
    \scalebox{0.78}{1.214} & \scalebox{0.78}{1.214} &
    \scalebox{0.78}{1.223} & \scalebox{0.78}{1.223} &
    \scalebox{0.78}{1.675} & \scalebox{0.78}{1.675} &
    \scalebox{0.78}{1.561} & \scalebox{0.78}{1.561} &
    \scalebox{0.78}{1.463} & \scalebox{0.78}{1.463} &
    \scalebox{0.78}{1.439} & \scalebox{0.78}{1.439} &
    \scalebox{0.78}{1.890} & \scalebox{0.78}{1.890} &
    \scalebox{0.78}{1.495} & \scalebox{0.78}{1.495} &
    \scalebox{0.78}{1.382} & \scalebox{0.78}{1.382} &
    \scalebox{0.78}{-} & \scalebox{0.78}{-} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \hline

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{SolarPower}}}

    & \scalebox{0.78}{96} &
    \scalebox{0.78}{0.010} & \scalebox{0.78}{0.031} &
    \scalebox{0.78}{0.011} & \scalebox{0.78}{0.032} &
    \scalebox{0.78}{0.011} & \scalebox{0.78}{0.032} &
    \scalebox{0.78}{0.016} & \scalebox{0.78}{0.043} &
    \scalebox{0.78}{0.013} & \scalebox{0.78}{0.037} &
    \scalebox{0.78}{0.014} & \scalebox{0.78}{0.041} &
    \scalebox{0.78}{0.013} & \scalebox{0.78}{0.039} &
    \scalebox{0.78}{0.012} & \scalebox{0.78}{0.033} &
    \scalebox{0.78}{0.017} & \scalebox{0.78}{0.045} &
    \scalebox{0.78}{0.015} & \scalebox{0.78}{0.041} &
    \scalebox{0.78}{0.013} & \scalebox{0.78}{0.039} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{192} &
    \scalebox{0.78}{0.020} & \scalebox{0.78}{0.048} &
    \scalebox{0.78}{0.020} & \scalebox{0.78}{0.049} &
    \scalebox{0.78}{0.020} & \scalebox{0.78}{0.049} &
    \scalebox{0.78}{0.025} & \scalebox{0.78}{0.058} &
    \scalebox{0.78}{0.022} & \scalebox{0.78}{0.053} &
    \scalebox{0.78}{0.023} & \scalebox{0.78}{0.055} &
    \scalebox{0.78}{0.023} & \scalebox{0.78}{0.055} &
    \scalebox{0.78}{0.021} & \scalebox{0.78}{0.050} &
    \scalebox{0.78}{0.024} & \scalebox{0.78}{0.057} &
    \scalebox{0.78}{0.023} & \scalebox{0.78}{0.056} &
    \scalebox{0.78}{0.024} & \scalebox{0.78}{0.058} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{336} &
    \scalebox{0.78}{0.032} & \scalebox{0.78}{0.067} &
    \scalebox{0.78}{0.032} & \scalebox{0.78}{0.067} &
    \scalebox{0.78}{0.032} & \scalebox{0.78}{0.068} &
    \scalebox{0.78}{0.036} & \scalebox{0.78}{0.074} &
    \scalebox{0.78}{0.034} & \scalebox{0.78}{0.071} &
    \scalebox{0.78}{0.035} & \scalebox{0.78}{0.072} &
    \scalebox{0.78}{0.034} & \scalebox{0.78}{0.072} &
    \scalebox{0.78}{0.033} & \scalebox{0.78}{0.068} &
    \scalebox{0.78}{0.036} & \scalebox{0.78}{0.074} &
    \scalebox{0.78}{0.034} & \scalebox{0.78}{0.072} &
    \scalebox{0.78}{0.037} & \scalebox{0.78}{0.075} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{720} &
    \scalebox{0.78}{0.063} & \scalebox{0.78}{0.104} &
    \scalebox{0.78}{0.063} & \scalebox{0.78}{0.105} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{0.068} & \scalebox{0.78}{0.110} &
    \scalebox{0.78}{0.066} & \scalebox{0.78}{0.108} &
    \scalebox{0.78}{0.067} & \scalebox{0.78}{0.110} &
    \scalebox{0.78}{0.065} & \scalebox{0.78}{0.108} &
    \scalebox{0.78}{0.064} & \scalebox{0.78}{0.104} &
    \scalebox{0.78}{0.068} & \scalebox{0.78}{0.110} &
    \scalebox{0.78}{0.065} & \scalebox{0.78}{0.107} &
    \scalebox{0.78}{0.068} & \scalebox{0.78}{0.110} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \cline{2-28}

    & \scalebox{0.78}{Avg} &
    \scalebox{0.78}{0.031} & \scalebox{0.78}{0.031} &
    \scalebox{0.78}{0.032} & \scalebox{0.78}{0.032} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{0.036} & \scalebox{0.78}{0.036} &
    \scalebox{0.78}{0.034} & \scalebox{0.78}{0.034} &
    \scalebox{0.78}{0.035} & \scalebox{0.78}{0.035} &
    \scalebox{0.78}{0.034} & \scalebox{0.78}{0.034} &
    \scalebox{0.78}{0.033} & \scalebox{0.78}{0.033} &
    \scalebox{0.78}{0.036} & \scalebox{0.78}{0.036} &
    \scalebox{0.78}{0.034} & \scalebox{0.78}{0.034} &
    \scalebox{0.78}{0.036} & \scalebox{0.78}{0.036} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \hline

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{WindPower}}}

    & \scalebox{0.78}{96} &
    \scalebox{0.78}{0.005} & \scalebox{0.78}{0.039} &
    \scalebox{0.78}{0.005} & \scalebox{0.78}{0.039} &
    \scalebox{0.78}{0.005} & \scalebox{0.78}{0.039} &
    \scalebox{0.78}{0.008} & \scalebox{0.78}{0.049} &
    \scalebox{0.78}{0.006} & \scalebox{0.78}{0.042} &
    \scalebox{0.78}{0.007} & \scalebox{0.78}{0.046} &
    \scalebox{0.78}{0.007} & \scalebox{0.78}{0.044} &
    \scalebox{0.78}{0.005} & \scalebox{0.78}{0.038} &
    \scalebox{0.78}{0.010} & \scalebox{0.78}{0.053} &
    \scalebox{0.78}{0.008} & \scalebox{0.78}{0.047} &
    \scalebox{0.78}{0.007} & \scalebox{0.78}{0.044} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{192} &
    \scalebox{0.78}{0.012} & \scalebox{0.78}{0.058} &
    \scalebox{0.78}{0.012} & \scalebox{0.78}{0.058} &
    \scalebox{0.78}{0.012} & \scalebox{0.78}{0.058} &
    \scalebox{0.78}{0.015} & \scalebox{0.78}{0.067} &
    \scalebox{0.78}{0.013} & \scalebox{0.78}{0.062} &
    \scalebox{0.78}{0.014} & \scalebox{0.78}{0.065} &
    \scalebox{0.78}{0.014} & \scalebox{0.78}{0.065} &
    \scalebox{0.78}{0.012} & \scalebox{0.78}{0.057} &
    \scalebox{0.78}{0.015} & \scalebox{0.78}{0.067} &
    \scalebox{0.78}{0.015} & \scalebox{0.78}{0.065} &
    \scalebox{0.78}{0.016} & \scalebox{0.78}{0.067} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{336} &
    \scalebox{0.78}{0.023} & \scalebox{0.78}{0.082} &
    \scalebox{0.78}{0.023} & \scalebox{0.78}{0.082} &
    \scalebox{0.78}{0.023} & \scalebox{0.78}{0.082} &
    \scalebox{0.78}{0.026} & \scalebox{0.78}{0.089} &
    \scalebox{0.78}{0.025} & \scalebox{0.78}{0.085} &
    \scalebox{0.78}{0.025} & \scalebox{0.78}{0.087} &
    \scalebox{0.78}{0.025} & \scalebox{0.78}{0.087} &
    \scalebox{0.78}{0.022} & \scalebox{0.78}{0.080} &
    \scalebox{0.78}{0.026} & \scalebox{0.78}{0.089} &
    \scalebox{0.78}{0.025} & \scalebox{0.78}{0.086} &
    \scalebox{0.78}{0.027} & \scalebox{0.78}{0.090} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    & \scalebox{0.78}{720} &
    \scalebox{0.78}{0.050} & \scalebox{0.78}{0.128} &
    \scalebox{0.78}{0.050} & \scalebox{0.78}{0.128} &
    \scalebox{0.78}{0.050} & \scalebox{0.78}{0.128} &
    \scalebox{0.78}{0.053} & \scalebox{0.78}{0.132} &
    \scalebox{0.78}{0.052} & \scalebox{0.78}{0.130} &
    \scalebox{0.78}{0.052} & \scalebox{0.78}{0.131} &
    \scalebox{0.78}{0.052} & \scalebox{0.78}{0.130} &
    \scalebox{0.78}{0.049} & \scalebox{0.78}{0.125} &
    \scalebox{0.78}{0.053} & \scalebox{0.78}{0.133} &
    \scalebox{0.78}{0.051} & \scalebox{0.78}{0.129} &
    \scalebox{0.78}{0.053} & \scalebox{0.78}{0.133} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \cline{2-28}

    & \scalebox{0.78}{Avg} &
    \scalebox{0.78}{0.022} & \scalebox{0.78}{0.022} &
    \scalebox{0.78}{0.022} & \scalebox{0.78}{0.022} &
    \scalebox{0.78}{0.022} & \scalebox{0.78}{0.022} &
    \scalebox{0.78}{0.026} & \scalebox{0.78}{0.026} &
    \scalebox{0.78}{0.024} & \scalebox{0.78}{0.024} &
    \scalebox{0.78}{0.025} & \scalebox{0.78}{0.025} &
    \scalebox{0.78}{0.025} & \scalebox{0.78}{0.025} &
    \scalebox{0.78}{0.022} & \scalebox{0.78}{0.022} &
    \scalebox{0.78}{0.026} & \scalebox{0.78}{0.026} &
    \scalebox{0.78}{0.025} & \scalebox{0.78}{0.025} &
    \scalebox{0.78}{0.026} & \scalebox{0.78}{0.026} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} &
    \scalebox{0.78}{*} & \scalebox{0.78}{*} \\

    \hline
    
    \multicolumn{2}{c}{\scalebox{0.76}{{$1^{\text{st}}$ Count}}} & 
    \multicolumn{6}{c}{\textbf{\scalebox{0.76}{0}}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} &  
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} \\
    
    \hline
  \end{tabular}
    \end{small}
  \end{threeparttable}
   }
\end{table*}

==> tables/forecasting_few_10_cross.tex <==
\begin{table*}[htpb]
  \caption{Long Forecasting (few-shot 10\%) \\ Cross-domain}\label{tab:forecasting_few_10_cross}
  \vspace{5pt}
  \centering
  \resizebox{2\columnwidth}{!}{
  \begin{small}
  \renewcommand{\multirowsetup}{\centering}
  \setlength{\tabcolsep}{1.5pt}
  \renewcommand\arraystretch{1.2}
  \begin{tabular}{cccc|cc||cccccccccccc}
    \toprule
    
    \multicolumn{2}{c}{\multirow{2}{*}{\scalebox{1.0}{Scenarios}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\textbf{CWT}}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Random init.}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{GPT4TS}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{DLinear}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{PatchTST}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimesNet}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{FEDformer}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Autoformer}}} \\

    % \multicolumn{2}{c}{} & 
    % \multicolumn{2}{c}{\scalebox{0.8}{(\textbf{Ours})}} & 
    % \multicolumn{2}{c}{\scalebox{0.8}{(\textbf{Ours})}} & 
    % \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{Nie2023ATS}}} &
    % \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wu2023timesnet}}} &
    % \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wang2023micn}}} &
    % \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{Zhang2022LessIM}}} &
    % \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{Zeng2022AreTE}}} & 
    % \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{zhou2022fedformer}}} \\
    
    \cmidrule(lr){3-18} &  & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} \\
    \toprule
    
    \multirow{5}{*}{\scalebox{0.9}{\shortstack{ETTm2\\ $\downarrow$ \\ETTm1}}}
    
    & \scalebox{0.78}{96} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{192} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{336} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    & \scalebox{0.78}{720} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \cmidrule(lr){2-18}

    & \scalebox{0.78}{avg} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \midrule
    
    \multirow{5}{*}{\scalebox{0.9}{\shortstack{ETTm1\\ $\downarrow$ \\ETTm2}}}
    
    & \scalebox{0.78}{96} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{192} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{336} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    & \scalebox{0.78}{720} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \cmidrule(lr){2-18}

    & \scalebox{0.78}{avg} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \midrule
    
    \multirow{5}{*}{\scalebox{0.9}{\shortstack{ETTh2\\ $\downarrow$ \\ETTh1}}}
    
    & \scalebox{0.78}{96} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{192} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{336} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    & \scalebox{0.78}{720} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \cmidrule(lr){2-18}

    & \scalebox{0.78}{avg} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \midrule
    
    \multirow{5}{*}{\scalebox{0.9}{\shortstack{ETTh1\\ $\downarrow$ \\ETTh2}}}
    
    & \scalebox{0.78}{96} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{192} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{336} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    & \scalebox{0.78}{720} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \cmidrule(lr){2-18}

    & \scalebox{0.78}{avg} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \midrule
    
    \multirow{5}{*}{\scalebox{0.9}{\shortstack{RiverFlow\\ $\downarrow$ \\Exchange}}}
    
    & \scalebox{0.78}{96} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{192} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{336} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    & \scalebox{0.78}{720} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \cmidrule(lr){2-18}

    & \scalebox{0.78}{avg} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \midrule
    
    \multirow{5}{*}{\scalebox{0.9}{\shortstack{Sunspot\\ $\downarrow$ \\Weather}}}
    
    & \scalebox{0.78}{96} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{192} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{336} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    & \scalebox{0.78}{720} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \cmidrule(lr){2-18}

    & \scalebox{0.78}{avg} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \bottomrule
    \bottomrule
  \end{tabular}
  \end{small}
}
\end{table*}

==> tables/forecasting_few_5_cross.tex <==
\begin{table*}[htpb]
  \caption{Long Forecasting (few-shot 5\%) \\ Cross-domain}\label{tab:forecasting_few_5_cross}
  \vspace{5pt}
  \centering
  \resizebox{2\columnwidth}{!}{
  \begin{small}
  \renewcommand{\multirowsetup}{\centering}
  \setlength{\tabcolsep}{1.5pt}
  \renewcommand\arraystretch{1.2}
  \begin{tabular}{cccc|cc||cccccccccccc}
    \toprule
    
    \multicolumn{2}{c}{\multirow{2}{*}{\scalebox{1.0}{Scenarios}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{\textbf{CWT}}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Random init.}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{GPT4TS}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{DLinear}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{PatchTST}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{TimesNet}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{FEDformer}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Autoformer}}} \\

    % \multicolumn{2}{c}{} & 
    % \multicolumn{2}{c}{\scalebox{0.8}{(\textbf{Ours})}} & 
    % \multicolumn{2}{c}{\scalebox{0.8}{(\textbf{Ours})}} & 
    % \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{Nie2023ATS}}} &
    % \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wu2023timesnet}}} &
    % \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{wang2023micn}}} &
    % \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{Zhang2022LessIM}}} &
    % \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{Zeng2022AreTE}}} & 
    % \multicolumn{2}{c}{\scalebox{0.8}{\citeyear{zhou2022fedformer}}} \\
    
    \cmidrule(lr){3-18} &  & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} & 
    \scalebox{0.78}{MSE} & \scalebox{0.78}{MAE} \\
    \toprule
    
    \multirow{5}{*}{\scalebox{0.9}{\shortstack{ETTm2\\ $\downarrow$ \\ETTm1}}}
    
    & \scalebox{0.78}{96} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{192} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{336} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    & \scalebox{0.78}{720} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \cmidrule(lr){2-18}

    & \scalebox{0.78}{avg} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \midrule
    
    \multirow{5}{*}{\scalebox{0.9}{\shortstack{ETTm1\\ $\downarrow$ \\ETTm2}}}
    
    & \scalebox{0.78}{96} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{192} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{336} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    & \scalebox{0.78}{720} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \cmidrule(lr){2-18}

    & \scalebox{0.78}{avg} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \midrule
    
    \multirow{5}{*}{\scalebox{0.9}{\shortstack{ETTh2\\ $\downarrow$ \\ETTh1}}}
    
    & \scalebox{0.78}{96} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{192} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{336} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    & \scalebox{0.78}{720} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} \\

    \cmidrule(lr){2-18}

    & \scalebox{0.78}{avg} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \midrule
    
    \multirow{5}{*}{\scalebox{0.9}{\shortstack{ETTh1\\ $\downarrow$ \\ETTh2}}}
    
    & \scalebox{0.78}{96} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{192} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{336} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    & \scalebox{0.78}{720} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} & 
    {\scalebox{0.78}{-}} & {\scalebox{0.78}{-}} \\

    \cmidrule(lr){2-18}

    & \scalebox{0.78}{avg} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \midrule
    
    \multirow{5}{*}{\scalebox{0.9}{\shortstack{RiverFlow\\ $\downarrow$ \\Exchange}}}
    
    & \scalebox{0.78}{96} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{192} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{336} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    & \scalebox{0.78}{720} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \cmidrule(lr){2-18}

    & \scalebox{0.78}{avg} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \midrule
    
    \multirow{5}{*}{\scalebox{0.9}{\shortstack{Sunspot\\ $\downarrow$ \\Weather}}}
    
    & \scalebox{0.78}{96} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{192} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\
    
    & \scalebox{0.78}{336} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    & \scalebox{0.78}{720} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \cmidrule(lr){2-18}

    & \scalebox{0.78}{avg} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} & 
    {\scalebox{0.78}{0.000}} & {\scalebox{0.78}{0.000}} \\

    \bottomrule
    \bottomrule
  \end{tabular}
  \end{small}
}
\end{table*}

==> tables/imputation.tex <==
\begin{table*}[htbp]
  \caption{CWT-adapter in Imputation (cross-zero) Task.\\ Imputation2Imputation}\label{tab:imputation}
  \vskip 0.05in
  \centering
  \resizebox{2\columnwidth}{!}{
  \begin{threeparttable}
  \begin{small}
  \renewcommand{\multirowsetup}{\centering}
  \setlength{\tabcolsep}{0.8pt}
  \begin{tabular}{c|c|cc|cc|cc||cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}

    \hline
    \hline
    \multicolumn{2}{c}{\multirow{1}{*}{Source}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Scratch-1.0}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Scratch-0.1}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Scratch-0.05}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{ETTm1}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{ETTm2}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{ETTh1}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{ETTh2}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Exchange}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Weather}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{Sunspot}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{RiverFlow}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{SolarPower}}} & 
    \multicolumn{2}{c}{\rotatebox{0}{\scalebox{0.8}{WindPower}}} \\
    
    \hline
    
    \multicolumn{2}{c}{\scalebox{0.76}{MaskRatio}} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} & 
    \scalebox{0.76}{MSE} & \scalebox{0.76}{MAE} \\
    
    \hline
    
    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ETTm1}}}
    
    & \scalebox{0.76}{12.5\%} &
    \scalebox{0.78}{0.037} &\scalebox{0.78}{0.123} &
    \scalebox{0.78}{0.062} &\scalebox{0.78}{0.166} &
    \scalebox{0.78}{0.094} &\scalebox{0.78}{0.204} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.043} &\scalebox{0.78}{0.134} &
    \scalebox{0.78}{0.057} &\scalebox{0.78}{0.156} &
    \scalebox{0.78}{0.054} &\scalebox{0.78}{0.154} &
    \scalebox{0.78}{0.065} &\scalebox{0.78}{0.167} &
    \scalebox{0.76}{0.046} &\scalebox{0.76}{0.140} & 
    \scalebox{0.78}{0.602} &\scalebox{0.78}{0.503} &
    \scalebox{0.78}{0.604} &\scalebox{0.78}{0.503} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{25\%} &
    \scalebox{0.78}{0.038} &\scalebox{0.78}{0.124} &
    \scalebox{0.78}{0.064} &\scalebox{0.78}{0.169} &
    \scalebox{0.78}{0.099} &\scalebox{0.78}{0.209} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.046} &\scalebox{0.78}{0.139} &
    \scalebox{0.78}{0.061} &\scalebox{0.78}{0.161} &
    \scalebox{0.78}{0.055} &\scalebox{0.78}{0.155} &
    \scalebox{0.78}{0.064} &\scalebox{0.78}{0.166} &
    \scalebox{0.78}{0.090} &\scalebox{0.78}{0.197} &
    \scalebox{0.78}{0.600} &\scalebox{0.78}{0.502} &
    \scalebox{0.78}{0.602} &\scalebox{0.78}{0.502} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{37.5\%} &
    \scalebox{0.78}{0.042} &\scalebox{0.78}{0.132} &
    \scalebox{0.78}{0.072} &\scalebox{0.78}{0.178} &
    \scalebox{0.78}{0.112} &\scalebox{0.78}{0.222} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.050} &\scalebox{0.78}{0.145} &
    \scalebox{0.78}{0.067} &\scalebox{0.78}{0.168} &
    \scalebox{0.78}{0.063} &\scalebox{0.78}{0.166} &
    \scalebox{0.78}{0.064} &\scalebox{0.78}{0.166} &
    \scalebox{0.78}{0.091} &\scalebox{0.78}{0.198} &
    \scalebox{0.78}{0.601} &\scalebox{0.78}{0.502} &
    \scalebox{0.78}{0.461} &\scalebox{0.78}{0.431} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{50\%} &
    \scalebox{0.78}{0.046} &\scalebox{0.78}{0.136} &
    \scalebox{0.78}{0.081} &\scalebox{0.78}{0.190} &
    \scalebox{0.78}{0.119} &\scalebox{0.78}{0.229} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.061} &\scalebox{0.78}{0.159} &
    \scalebox{0.78}{0.089} &\scalebox{0.78}{0.193} &
    \scalebox{0.78}{0.073} &\scalebox{0.78}{0.177} &
    \scalebox{0.78}{0.075} &\scalebox{0.78}{0.178} &
    \scalebox{0.78}{0.075} &\scalebox{0.78}{0.179} &
    \scalebox{0.78}{0.604} &\scalebox{0.78}{0.503} &
    \scalebox{0.78}{0.605} &\scalebox{0.78}{0.504} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \cline{2-28}
    
    & \scalebox{0.76}{Avg} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \hline
    
    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ETTm2}}} 

    & \scalebox{0.76}{12.5\%} &
    \scalebox{0.78}{0.025} &\scalebox{0.78}{0.092} &
    \scalebox{0.78}{0.039} &\scalebox{0.78}{0.123} &
    \scalebox{0.78}{0.046} &\scalebox{0.78}{0.136} &
    \scalebox{0.78}{0.026} &\scalebox{0.78}{0.094} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.029} &\scalebox{0.78}{0.103} &
    \scalebox{0.76}{0.031} &\scalebox{0.76}{0.107} & 
    \scalebox{0.78}{0.034} &\scalebox{0.78}{0.111} &
    \scalebox{0.78}{0.029} &\scalebox{0.78}{0.100} &
    \scalebox{0.78}{0.119} &\scalebox{0.78}{0.235} &
    \scalebox{0.78}{0.120} &\scalebox{0.78}{0.235} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{25\%} &
    \scalebox{0.78}{0.027} &\scalebox{0.78}{0.095} &
    \scalebox{0.78}{0.041} &\scalebox{0.78}{0.126} &
    \scalebox{0.78}{0.047} &\scalebox{0.78}{0.138} &
    \scalebox{0.78}{0.028} &\scalebox{0.78}{0.095} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.030} &\scalebox{0.78}{0.106} &
    \scalebox{0.76}{0.032} &\scalebox{0.76}{0.108} & 
    \scalebox{0.78}{0.034} &\scalebox{0.78}{0.111} &
    \scalebox{0.78}{0.039} &\scalebox{0.78}{0.121} &
    \scalebox{0.78}{0.119} &\scalebox{0.78}{0.235} &
    \scalebox{0.78}{0.120} &\scalebox{0.78}{0.235} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{37.5\%} &
    \scalebox{0.76}{0.028} &\scalebox{0.76}{0.098} & 
    \scalebox{0.78}{0.043} &\scalebox{0.78}{0.129} &
    \scalebox{0.78}{0.051} &\scalebox{0.78}{0.144} &
    \scalebox{0.78}{0.030} &\scalebox{0.78}{0.100} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.033} &\scalebox{0.78}{0.110} &
    \scalebox{0.76}{0.035} &\scalebox{0.76}{0.114} & 
    \scalebox{0.78}{0.035} &\scalebox{0.78}{0.112} &
    \scalebox{0.78}{0.040} &\scalebox{0.78}{0.123} &
    \scalebox{0.78}{0.120} &\scalebox{0.78}{0.235} &
    \scalebox{0.78}{0.090} &\scalebox{0.78}{0.201} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{50\%} &
    \scalebox{0.76}{0.032} &\scalebox{0.76}{0.105} & 
    \scalebox{0.78}{0.047} &\scalebox{0.78}{0.135} &
    \scalebox{0.78}{0.055} &\scalebox{0.78}{0.151} &
    \scalebox{0.78}{0.033} &\scalebox{0.78}{0.104} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.038} &\scalebox{0.78}{0.120} &
    \scalebox{0.76}{0.038} &\scalebox{0.76}{0.119} & 
    \scalebox{0.78}{0.038} &\scalebox{0.78}{0.118} &
    \scalebox{0.78}{0.039} &\scalebox{0.78}{0.118} &
    \scalebox{0.78}{0.120} &\scalebox{0.78}{0.236} &
    \scalebox{0.78}{0.120} &\scalebox{0.78}{0.236} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \cline{2-28}
    
    & \scalebox{0.76}{Avg} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \hline
    
    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ETTh1}}} 
    
    & \scalebox{0.76}{12.5\%} &
    \scalebox{0.78}{0.100} &\scalebox{0.78}{0.214} &
    \scalebox{0.78}{0.306} &\scalebox{0.78}{0.370} &
    \scalebox{0.78}{0.455} &\scalebox{0.78}{0.441} &
    \scalebox{0.78}{0.147} &\scalebox{0.78}{0.255} &
    \scalebox{0.78}{0.128} &\scalebox{0.78}{0.241} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.184} &\scalebox{0.78}{0.281} &
    \scalebox{0.78}{0.346} &\scalebox{0.78}{0.378} &
    \scalebox{0.78}{0.242} &\scalebox{0.78}{0.318} &
    \scalebox{0.78}{0.652} &\scalebox{0.78}{0.532} &
    \scalebox{0.78}{0.653} &\scalebox{0.78}{0.533} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{25\%} &
    \scalebox{0.78}{0.110} &\scalebox{0.78}{0.224} &
    \scalebox{0.78}{0.316} &\scalebox{0.78}{0.376} &
    \scalebox{0.78}{0.456} &\scalebox{0.78}{0.443} &
    \scalebox{0.78}{0.161} &\scalebox{0.78}{0.265} &
    \scalebox{0.78}{0.148} &\scalebox{0.78}{0.257} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.192} &\scalebox{0.78}{0.286} &
    \scalebox{0.78}{0.336} &\scalebox{0.78}{0.371} &
    \scalebox{0.78}{0.425} &\scalebox{0.78}{0.418} &
    \scalebox{0.78}{0.653} &\scalebox{0.78}{0.533} &
    \scalebox{0.78}{0.654} &\scalebox{0.78}{0.533} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{37.5\%} &
    \scalebox{0.78}{0.124} &\scalebox{0.78}{0.237} &
    \scalebox{0.78}{0.351} &\scalebox{0.78}{0.395} &
    \scalebox{0.78}{0.481} &\scalebox{0.78}{0.453} &
    \scalebox{0.78}{0.203} &\scalebox{0.78}{0.294} &
    \scalebox{0.78}{0.183} &\scalebox{0.78}{0.283} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.222} &\scalebox{0.78}{0.307} &
    \scalebox{0.78}{0.340} &\scalebox{0.78}{0.372} &
    \scalebox{0.76}{0.477} &\scalebox{0.76}{0.442} & 
    \scalebox{0.78}{0.655} &\scalebox{0.78}{0.534} &
    \scalebox{0.78}{0.639} &\scalebox{0.78}{0.524} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{50\%} &
    \scalebox{0.78}{0.156} &\scalebox{0.78}{0.265} &
    \scalebox{0.78}{0.444} &\scalebox{0.78}{0.438} &
    \scalebox{0.78}{0.516} &\scalebox{0.78}{0.469} &
    \scalebox{0.78}{0.244} &\scalebox{0.78}{0.317} &
    \scalebox{0.78}{0.249} &\scalebox{0.78}{0.323} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.268} &\scalebox{0.78}{0.335} &
    \scalebox{0.78}{0.404} &\scalebox{0.78}{0.406} &
    \scalebox{0.78}{0.529} &\scalebox{0.78}{0.466} &
    \scalebox{0.78}{0.658} &\scalebox{0.78}{0.535} &
    \scalebox{0.78}{0.659} &\scalebox{0.78}{0.536} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \cline{2-28}
    
    & \scalebox{0.76}{Avg} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \hline
    
    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{ETTh2}}}
    
    & \scalebox{0.76}{12.5\%} &
    \scalebox{0.78}{0.063} &\scalebox{0.78}{0.161} &
    \scalebox{0.78}{0.113} &\scalebox{0.78}{0.227} &
    \scalebox{0.78}{0.132} &\scalebox{0.78}{0.245} &
    \scalebox{0.78}{0.059} &\scalebox{0.78}{0.152} &
    \scalebox{0.76}{0.059} &\scalebox{0.76}{0.152} & 
    \scalebox{0.78}{0.059} &\scalebox{0.78}{0.152} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.079} &\scalebox{0.78}{0.186} &
    \scalebox{0.78}{0.066} &\scalebox{0.78}{0.166} &
    \scalebox{0.78}{0.189} &\scalebox{0.78}{0.297} &
    \scalebox{0.78}{0.189} &\scalebox{0.78}{0.297} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{25\%} &
    \scalebox{0.78}{0.064} &\scalebox{0.78}{0.162} &
    \scalebox{0.78}{0.113} &\scalebox{0.78}{0.227} &
    \scalebox{0.78}{0.128} &\scalebox{0.78}{0.241} &
    \scalebox{0.78}{0.062} &\scalebox{0.78}{0.155} &
    \scalebox{0.76}{0.062} &\scalebox{0.76}{0.158} & 
    \scalebox{0.78}{0.061} &\scalebox{0.78}{0.156} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.079} &\scalebox{0.78}{0.185} &
    \scalebox{0.78}{0.091} &\scalebox{0.78}{0.203} &
    \scalebox{0.78}{0.191} &\scalebox{0.78}{0.297} &
    \scalebox{0.78}{0.191} &\scalebox{0.78}{0.298} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{37.5\%} &
    \scalebox{0.78}{0.069} &\scalebox{0.78}{0.170} &
    \scalebox{0.78}{0.125} &\scalebox{0.78}{0.239} &
    \scalebox{0.78}{0.136} &\scalebox{0.78}{0.249} &
    \scalebox{0.78}{0.068} &\scalebox{0.78}{0.164} &
    \scalebox{0.76}{0.067} &\scalebox{0.76}{0.165} & 
    \scalebox{0.78}{0.065} &\scalebox{0.78}{0.161} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.080} &\scalebox{0.78}{0.186} &
    \scalebox{0.78}{0.092} &\scalebox{0.78}{0.205} &
    \scalebox{0.78}{0.191} &\scalebox{0.78}{0.297} &
    \scalebox{0.78}{0.155} &\scalebox{0.78}{0.270} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{50\%} &
    \scalebox{0.78}{0.076} &\scalebox{0.78}{0.179} &
    \scalebox{0.78}{0.146} &\scalebox{0.78}{0.259} &
    \scalebox{0.78}{0.151} &\scalebox{0.78}{0.263} &
    \scalebox{0.78}{0.073} &\scalebox{0.78}{0.171} &
    \scalebox{0.76}{0.075} &\scalebox{0.76}{0.177} & 
    \scalebox{0.78}{0.072} &\scalebox{0.78}{0.172} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.089} &\scalebox{0.78}{0.198} &
    \scalebox{0.78}{0.094} &\scalebox{0.78}{0.206} &
    \scalebox{0.78}{0.192} &\scalebox{0.78}{0.298} &
    \scalebox{0.78}{0.192} &\scalebox{0.78}{0.298} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \cline{2-28}
    
    & \scalebox{0.76}{Avg} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \hline
    
    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{Exchange}}}
    
    & \scalebox{0.76}{12.5\%} &
    \scalebox{0.78}{0.003} &\scalebox{0.78}{0.037} &
    \scalebox{0.78}{0.011} &\scalebox{0.78}{0.068} &
    \scalebox{0.78}{0.015} &\scalebox{0.78}{0.084} &
    \scalebox{0.78}{0.003} &\scalebox{0.78}{0.029} &
    \scalebox{0.76}{0.004} &\scalebox{0.76}{0.029} & 
    \scalebox{0.78}{0.004} &\scalebox{0.78}{0.033} &
    \scalebox{0.76}{0.005} &\scalebox{0.76}{0.035} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.004} &\scalebox{0.78}{0.032} &
    \scalebox{0.78}{0.028} &\scalebox{0.78}{0.118} &
    \scalebox{0.78}{0.029} &\scalebox{0.78}{0.119} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{25\%} &
    \scalebox{0.78}{0.004} &\scalebox{0.78}{0.037} &
    \scalebox{0.78}{0.011} &\scalebox{0.78}{0.071} &
    \scalebox{0.78}{0.016} &\scalebox{0.78}{0.085} &
    \scalebox{0.78}{0.003} &\scalebox{0.78}{0.029} &
    \scalebox{0.76}{0.004} &\scalebox{0.76}{0.030} & 
    \scalebox{0.78}{0.004} &\scalebox{0.78}{0.035} &
    \scalebox{0.76}{0.004} &\scalebox{0.76}{0.036} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.005} &\scalebox{0.78}{0.043} &
    \scalebox{0.78}{0.028} &\scalebox{0.78}{0.118} &
    \scalebox{0.78}{0.028} &\scalebox{0.78}{0.118} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{37.5\%} &
    \scalebox{0.78}{0.004} &\scalebox{0.78}{0.037} &
    \scalebox{0.78}{0.012} &\scalebox{0.78}{0.074} &
    \scalebox{0.78}{0.017} &\scalebox{0.78}{0.088} &
    \scalebox{0.78}{0.003} &\scalebox{0.78}{0.032} &
    \scalebox{0.76}{0.004} &\scalebox{0.76}{0.032} & 
    \scalebox{0.78}{0.004} &\scalebox{0.78}{0.036} &
    \scalebox{0.76}{0.005} &\scalebox{0.76}{0.038} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.006} &\scalebox{0.78}{0.045} &
    \scalebox{0.78}{0.028} &\scalebox{0.78}{0.118} &
    \scalebox{0.78}{0.015} &\scalebox{0.78}{0.082} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{50\%} &
    \scalebox{0.78}{0.005} &\scalebox{0.78}{0.040} &
    \scalebox{0.78}{0.013} &\scalebox{0.78}{0.078} &
    \scalebox{0.78}{0.018} &\scalebox{0.78}{0.092} &
    \scalebox{0.78}{0.004} &\scalebox{0.78}{0.033} &
    \scalebox{0.76}{0.004} &\scalebox{0.76}{0.035} & 
    \scalebox{0.78}{0.005} &\scalebox{0.78}{0.041} &
    \scalebox{0.76}{0.005} &\scalebox{0.76}{0.041} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.005} &\scalebox{0.78}{0.041} &
    \scalebox{0.78}{0.027} &\scalebox{0.78}{0.118} &
    \scalebox{0.78}{0.028} &\scalebox{0.78}{0.118} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \cline{2-28}
    
    & \scalebox{0.76}{Avg} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \hline
    
    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{Weather}}}
    
    & \scalebox{0.76}{12.5\%} &
    \scalebox{0.78}{0.029} &\scalebox{0.78}{0.044} &
    \scalebox{0.78}{0.041} &\scalebox{0.78}{0.063} &
    \scalebox{0.78}{0.049} &\scalebox{0.78}{0.078} &
    \scalebox{0.78}{0.028} &\scalebox{0.78}{0.041} &
    \scalebox{0.78}{0.027} &\scalebox{0.78}{0.041} &
    \scalebox{0.78}{0.030} &\scalebox{0.78}{0.049} &
    \scalebox{0.78}{0.032} &\scalebox{0.78}{0.051} &
    \scalebox{0.78}{0.034} &\scalebox{0.78}{0.051} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.102} &\scalebox{0.78}{0.159} &
    \scalebox{0.78}{0.102} &\scalebox{0.78}{0.159} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{25\%} &
    \scalebox{0.78}{0.030} &\scalebox{0.78}{0.046} &
    \scalebox{0.78}{0.042} &\scalebox{0.78}{0.065} &
    \scalebox{0.78}{0.049} &\scalebox{0.78}{0.076} &
    \scalebox{0.78}{0.029} &\scalebox{0.78}{0.041} &
    \scalebox{0.78}{0.029} &\scalebox{0.78}{0.043} &
    \scalebox{0.78}{0.032} &\scalebox{0.78}{0.051} &
    \scalebox{0.78}{0.033} &\scalebox{0.78}{0.051} &
    \scalebox{0.78}{0.034} &\scalebox{0.78}{0.051} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.102} &\scalebox{0.78}{0.160} &
    \scalebox{0.78}{0.102} &\scalebox{0.78}{0.160} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{37.5\%} &
    \scalebox{0.78}{0.032} &\scalebox{0.78}{0.049} &
    \scalebox{0.78}{0.045} &\scalebox{0.78}{0.068} &
    \scalebox{0.78}{0.050} &\scalebox{0.78}{0.077} &
    \scalebox{0.78}{0.032} &\scalebox{0.78}{0.044} &
    \scalebox{0.78}{0.031} &\scalebox{0.78}{0.045} &
    \scalebox{0.78}{0.034} &\scalebox{0.78}{0.054} &
    \scalebox{0.78}{0.035} &\scalebox{0.78}{0.055} &
    \scalebox{0.78}{0.035} &\scalebox{0.78}{0.052} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.103} &\scalebox{0.78}{0.160} &
    \scalebox{0.78}{0.076} &\scalebox{0.78}{0.121} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{50\%} &
    \scalebox{0.78}{0.035} &\scalebox{0.78}{0.050} &
    \scalebox{0.78}{0.048} &\scalebox{0.78}{0.072} &
    \scalebox{0.78}{0.050} &\scalebox{0.78}{0.076} &
    \scalebox{0.78}{0.034} &\scalebox{0.78}{0.046} &
    \scalebox{0.78}{0.034} &\scalebox{0.78}{0.049} &
    \scalebox{0.78}{0.038} &\scalebox{0.78}{0.060} &
    \scalebox{0.78}{0.038} &\scalebox{0.78}{0.058} &
    \scalebox{0.78}{0.038} &\scalebox{0.78}{0.055} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.103} &\scalebox{0.78}{0.160} &
    \scalebox{0.78}{0.103} &\scalebox{0.78}{0.160} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \cline{2-28}
    
    & \scalebox{0.76}{Avg} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \hline

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{Sunspot}}}
    
    & \scalebox{0.76}{12.5\%} &
    \scalebox{0.78}{0.259} &\scalebox{0.78}{0.361} &
    \scalebox{0.78}{0.260} &\scalebox{0.78}{0.361} &
    \scalebox{0.78}{0.260} &\scalebox{0.78}{0.361} &
    \scalebox{0.78}{0.039} &\scalebox{0.78}{0.142} &
    \scalebox{0.78}{0.042} &\scalebox{0.78}{0.144} &
    \scalebox{0.78}{0.049} &\scalebox{0.78}{0.156} &
    \scalebox{0.78}{0.070} &\scalebox{0.78}{0.187} &
    \scalebox{0.78}{0.097} &\scalebox{0.78}{0.217} &
    \scalebox{0.78}{0.057} &\scalebox{0.78}{0.169} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.259} &\scalebox{0.78}{0.36} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{25\%} &
    \scalebox{0.78}{0.261} &\scalebox{0.78}{0.361} &
    \scalebox{0.78}{0.261} &\scalebox{0.78}{0.362} &
    \scalebox{0.78}{0.261} &\scalebox{0.78}{0.361} &
    \scalebox{0.78}{0.043} &\scalebox{0.78}{0.146} &
    \scalebox{0.78}{0.049} &\scalebox{0.78}{0.155} &
    \scalebox{0.78}{0.055} &\scalebox{0.78}{0.165} &
    \scalebox{0.78}{0.072} &\scalebox{0.78}{0.189} &
    \scalebox{0.78}{0.094} &\scalebox{0.78}{0.213} &
    \scalebox{0.78}{0.122} &\scalebox{0.78}{0.244} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.261} &\scalebox{0.78}{0.361} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{37.5\%} &
    \scalebox{0.78}{0.261} &\scalebox{0.78}{0.361} &
    \scalebox{0.78}{0.261} &\scalebox{0.78}{0.362} &
    \scalebox{0.78}{0.261} &\scalebox{0.78}{0.362} &
    \scalebox{0.78}{0.054} &\scalebox{0.78}{0.163} &
    \scalebox{0.78}{0.059} &\scalebox{0.78}{0.170} &
    \scalebox{0.78}{0.063} &\scalebox{0.78}{0.176} &
    \scalebox{0.78}{0.087} &\scalebox{0.78}{0.207} &
    \scalebox{0.78}{0.093} &\scalebox{0.78}{0.212} &
    \scalebox{0.78}{0.124} &\scalebox{0.78}{0.246} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.237} &\scalebox{0.78}{0.342} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{50\%} &
    \scalebox{0.78}{0.263} &\scalebox{0.78}{0.363} &
    \scalebox{0.78}{0.263} &\scalebox{0.78}{0.363} &
    \scalebox{0.78}{0.263} &\scalebox{0.78}{0.362} &
    \scalebox{0.78}{0.063} &\scalebox{0.78}{0.174} &
    \scalebox{0.78}{0.079} &\scalebox{0.78}{0.196} &
    \scalebox{0.78}{0.084} &\scalebox{0.78}{0.202} &
    \scalebox{0.78}{0.101} &\scalebox{0.78}{0.222} &
    \scalebox{0.78}{0.113} &\scalebox{0.78}{0.233} &
    \scalebox{0.78}{0.109} &\scalebox{0.78}{0.230} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{0.263} &\scalebox{0.78}{0.362} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \cline{2-28}
    
    & \scalebox{0.76}{Avg} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\

    \hline

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{RiverFlow}}}
    
    & \scalebox{0.76}{12.5\%} &
    \scalebox{0.78}{0.913} &\scalebox{0.78}{0.495} &
    \scalebox{0.78}{0.889} &\scalebox{0.78}{0.491} &
    \scalebox{0.78}{0.924} &\scalebox{0.78}{0.495} &
    \scalebox{0.78}{0.141} &\scalebox{0.78}{0.165} &
    \scalebox{0.78}{0.139} &\scalebox{0.78}{0.169} &
    \scalebox{0.78}{0.178} &\scalebox{0.78}{0.193} &
    \scalebox{0.78}{0.240} &\scalebox{0.78}{0.229} &
    \scalebox{0.78}{0.301} &\scalebox{0.78}{0.247} &
    \scalebox{0.78}{0.163} &\scalebox{0.78}{0.187} &
    \scalebox{0.78}{0.909} &\scalebox{0.78}{0.493} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{25\%} &
    \scalebox{0.78}{0.936} &\scalebox{0.78}{0.496} &
    \scalebox{0.78}{0.928} &\scalebox{0.78}{0.494} &
    \scalebox{0.78}{0.905} &\scalebox{0.78}{0.495} &
    \scalebox{0.78}{0.151} &\scalebox{0.78}{0.166} &
    \scalebox{0.78}{0.157} &\scalebox{0.78}{0.176} &
    \scalebox{0.78}{0.197} &\scalebox{0.78}{0.200} &
    \scalebox{0.78}{0.241} &\scalebox{0.78}{0.229} &
    \scalebox{0.78}{0.291} &\scalebox{0.78}{0.240} &
    \scalebox{0.78}{0.335} &\scalebox{0.78}{0.273} &
    \scalebox{0.78}{0.905} &\scalebox{0.78}{0.493} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{37.5\%} &
    \scalebox{0.78}{0.755} &\scalebox{0.78}{0.425} &
    \scalebox{0.78}{0.908} &\scalebox{0.78}{0.493} &
    \scalebox{0.78}{0.907} &\scalebox{0.78}{0.494} &
    \scalebox{0.78}{0.187} &\scalebox{0.78}{0.185} &
    \scalebox{0.78}{0.190} &\scalebox{0.78}{0.194} &
    \scalebox{0.78}{0.226} &\scalebox{0.78}{0.212} &
    \scalebox{0.78}{0.284} &\scalebox{0.78}{0.249} &
    \scalebox{0.78}{0.295} &\scalebox{0.78}{0.242} &
    \scalebox{0.78}{0.349} &\scalebox{0.78}{0.284} &
    \scalebox{0.78}{0.912} &\scalebox{0.78}{0.496} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{50\%} &
    \scalebox{0.78}{0.919} &\scalebox{0.78}{0.493} &
    \scalebox{0.78}{0.912} &\scalebox{0.78}{0.494} &
    \scalebox{0.78}{0.916} &\scalebox{0.78}{0.494} &
    \scalebox{0.78}{0.215} &\scalebox{0.78}{0.195} &
    \scalebox{0.78}{0.244} &\scalebox{0.78}{0.219} &
    \scalebox{0.78}{0.285} &\scalebox{0.78}{0.241} &
    \scalebox{0.78}{0.322} &\scalebox{0.78}{0.264} &
    \scalebox{0.78}{0.338} &\scalebox{0.78}{0.258} &
    \scalebox{0.78}{0.318} &\scalebox{0.78}{0.242} &
    \scalebox{0.78}{0.915} &\scalebox{0.78}{0.495} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \cline{2-28}
    
    & \scalebox{0.76}{Avg} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\

    \hline
    
    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{SolarPower}}}
    
    & \scalebox{0.76}{12.5\%} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{25\%} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{37.5\%} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{50\%} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \cline{2-28}
    
    & \scalebox{0.76}{Avg} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\

    \hline

    \multirow{5}{*}{\rotatebox{90}{\scalebox{0.95}{WindPower}}}
    
    & \scalebox{0.76}{12.5\%} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{25\%} &
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{37.5\%} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    & \scalebox{0.76}{50\%} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\
    
    \cline{2-28}
    
    & \scalebox{0.76}{Avg} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.78}{-} &\scalebox{0.78}{-} &
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} & 
    \scalebox{0.76}{-} &\scalebox{0.76}{-} \\

    \hline
    
    \multicolumn{2}{c}{\scalebox{0.76}{{$1^{\text{st}}$ Count}}} & 
    \multicolumn{6}{c}{\textbf{\scalebox{0.76}{0}}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} &  
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} & 
    \multicolumn{2}{c}{\scalebox{0.76}{0}} \\
    
    \hline
  \end{tabular}
    \end{small}
  \end{threeparttable}
   }
\end{table*}

==> tables_brief/classification_few_raw.tex <==
\begin{table*}[htbp]
\caption{Classification (few-shot) (single-domain adaptation)}\label{tab:brief_classification_few_raw}
\vskip 0.1in
\centering
\resizebox{1.15\columnwidth}{!}{
\begin{threeparttable}
\begin{small}
\renewcommand{\multirowsetup}{\centering}
\setlength{\tabcolsep}{7pt}
\begin{tabular}{c|c|c|cccc|c}
\toprule
\hline

\multicolumn{2}{c}{Scenarios} & Models & Accuracy (\%) & Precision (\%) & Recall (\%) & F1 (\%) & Avg (\%) \\


\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{16}{*}[-3ex]{\rotatebox{90}{\shortstack{SonyAIBORobotSurface2 \\ $\downarrow$ \\ Chinatown}}}

& \multirow{4}{*}[0ex]{\shortstack{Full Data}}
& MICN & 63.27 & 55.17 & 55.49 & 55.27 & 57.30 \\
& & TimesNet & \textbf{97.96} & \textbf{96.53} & \textbf{98.59} & \textbf{97.49} & \textbf{97.64} \\
& & PatchTST & 95.63 & 94.38 & 94.67 & 94.52 & 94.80 \\
& & OneFitsAll & 96.79 & 94.94 & 97.46 & 96.08 & 96.32 \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (10\%)}}
& Random init. & 66.79 & 64.76 & 67.79 & 66.11 & 66.36 \\
\cmidrule(lr){3-8}
& & MICN & 27.41 & 13.70 & 50.00 & 21.51 & 28.15 \\
& & TimesNet & 91.25 & 89.65 & 88.02 & 88.78 & 89.43 \\
& & PatchTST & 80.76 & 87.95 & 65.22 & 67.52 & 75.36 \\
& & OneFitsAll & 78.13 & 74.21 & 65.40 & 67.21 & 71.24 \\
& & \myformer & \textbf{94.17} & \textbf{91.23} & \textbf{95.98} & \textbf{93.10} & \textbf{93.62} \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (5\%)}}
& Random init. & 27.41 & 13.70 & 50.00 & 21.51 & 28.16 \\
\cmidrule(lr){3-8}
& & MICN & 27.41 & 13.70 & 50.00 & 21.51 & 28.15 \\
& & TimesNet & 27.41 & 13.70 & 50.00 & 21.51 & 28.15 \\
& & PatchTST & 81.05 & 84.63 & 66.75 & 69.33 & 75.44 \\
& & OneFitsAll & 27.41 & 13.70 & 50.00 & 21.51 & 28.15 \\
& & \myformer & \textbf{91.55} & \textbf{90.16} & \textbf{88.22} & \textbf{89.12} & \textbf{89.76} \\


\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{16}{*}[-3ex]{\rotatebox{90}{\shortstack{HouseTwenty\\ $\downarrow$ \\ GunPointMaleVersusFemale}}}

& \multirow{4}{*}[0ex]{\shortstack{Full Data}}
& MICN & 98.73 & 98.77 & 98.70 & 98.73 & 98.73 \\
& & TimesNet & \textbf{99.05} & \textbf{99.07} & \textbf{99.03} & \textbf{99.05} & \textbf{99.05} \\
& & PatchTST & 97.47 & 97.44 & 97.49 & 97.46 & 97.47 \\
& & OneFitsAll & 94.62 & 95.00 & 94.37 & 93.24 & 94.31 \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (10\%)}}
& Random init. & 87.66 & 89.45 & 88.22 & 87.60 & 88.23 \\
\cmidrule(lr){3-8}
& & MICN & 75.63 & 78.43 & 76.39 & 75.33 & 76.44 \\
& & TimesNet & 81.96 & 82.73 & 81.55 & 81.68 & 81.98 \\
& & PatchTST & 96.84 & 96.80 & 96.89 & 96.83 & 96.84 \\
& & OneFitsAll & 76.27 & 78.42 & 76.93 & 76.06 & 76.92 \\
& & \myformer & \textbf{98.10} & \textbf{98.26} & \textbf{98.00} & \textbf{98.09} & \textbf{98.11} \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (5\%)}}
& Random init. & 66.77 & 69.86 & 67.67 & 66.08 & 67.59 \\
\cmidrule(lr){3-8}
& & MICN & 69.30 & 72.46 & 70.17 & 68.72 & 70.16 \\
& & TimesNet & 52.53 & 51.64 & 51.16 & 47.92 & 50.81 \\
& & PatchTST & 84.18 & 86.17 & 84.78 & 84.09 & 84.81 \\
& & OneFitsAll & 68.99 & 73.31 & 70.00 & 68.12 & 70.11 \\
& & \myformer & \textbf{85.76} & \textbf{85.79} & \textbf{85.64} & \textbf{85.70} & \textbf{85.72} \\


\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{16}{*}[-3ex]{\rotatebox{90}{\shortstack{PigArtPressure\\ $\downarrow$ \\ InsectEPGRegularTrain}}}

& \multirow{4}{*}[0ex]{\shortstack{Full Data}}
& MICN & \textbf{86.78} & 74.94 & \textbf{83.13} & \textbf{79.83} & \textbf{81.17} \\
& & TimesNet & 78.10 & 76.27 & 74.82 & 71.85 & 75.26 \\
& & PatchTST & 83.13 & \textbf{84.74} & 71.74 & 72.78 & 78.10 \\
& & OneFitsAll & 83.03 & 84.46 & 76.61 & 73.89 & 79.50 \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (10\%)}}
& Random init. & 47.39 & 15.80 & 33.33 & 21.44 & 29.49 \\
\cmidrule(lr){3-8}
& & MICN & 35.74 & 11.91 & 33.33 & 17.55 & 24.63 \\
& & TimesNet & 83.13 & 55.98 & 66.67 & 60.30 & 66.52 \\
& & PatchTST & 48.19 & 48.67 & 45.81 & 39.85 & 45.63 \\
& & OneFitsAll & 83.13 & 57.92 & 66.67 & 61.63 & 67.34 \\
& & \myformer & \textbf{93.17} & \textbf{93.74} & \textbf{87.53} & \textbf{89.68} & \textbf{91.03} \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (5\%)}}
& Random init. & 35.74 & 11.91 & 33.33 & 17.55 & 24.63 \\
\cmidrule(lr){3-8}
& & MICN & 35.74 & 11.91 & 33.33 & 17.55 & 24.63 \\
& & TimesNet & 35.74 & 15.86 & 33.33 & 21.50 & 26.61 \\
& & PatchTST & 37.35 & 20.95 & 37.35 & 24.50 & 30.04 \\
& & OneFitsAll & 35.74 & 11.91 & 33.33 & 17.55 & 24.63 \\
& & \myformer & \textbf{83.85} & \textbf{84.37} & \textbf{78.78} & \textbf{80.71} & \textbf{81.93} \\


\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{16}{*}[-3ex]{\rotatebox{90}{\shortstack{Earthquakes \\ $\downarrow$ \\ ItalyPowerDemand}}}

& \multirow{4}{*}[0ex]{\shortstack{Full Data}}
& MICN & 95.63 & 95.63 & 95.63 & 95.63 & 95.63 \\
& & TimesNet & \textbf{97.18} & \textbf{97.18} & \textbf{97.18} & \textbf{97.18} & \textbf{97.18} \\
& & PatchTST & 96.60 & 96.62 & 96.60 & 96.60 & 96.61 \\
& & OneFitsAll & 96.99 & 96.99 & 96.99 & 96.99 & 96.99 \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (10\%)}}
& Random init. & 78.92 & 79.58 & 78.90 & 78.87 & 79.07 \\
\cmidrule(lr){3-8}
& & MICN & 90.28 & 91.24 & 90.26 & 90.22 & 90.50 \\
& & TimesNet & 86.59 & 87.02 & 86.60 & 86.55 & 86.69 \\
& & PatchTST & 87.37 & 88.40 & 87.34 & 87.28 & 87.59 \\
& & OneFitsAll & 94.66 & 94.75 & 94.65 & 94.65 & 94.68 \\
& & \myformer & \textbf{96.31} & \textbf{96.34} & \textbf{96.30} & \textbf{96.31} & \textbf{96.31} \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (5\%)}}
& Random init. & 70.86 & 72.47 & 70.89 & 70.63 & 71.21 \\
\cmidrule(lr){3-8}
& & MICN & 70.94 & 77.75 & 71.01 & 69.09 & 72.19 \\
& & TimesNet & 73.28 & 77.08 & 73.33 & 72.33 & 74.01 \\
& & PatchTST & 60.93 & 64.96 & 61.01 & 58.20 & 61.27 \\
& & OneFitsAll & 83.19 & 85.25 & 83.22 & 82.95 & 83.65 \\
& & \myformer & \textbf{94.85} & \textbf{94.85} & \textbf{94.85} & \textbf{94.85} & \textbf{94.85} \\


\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{16}{*}[-3ex]{\rotatebox{90}{\shortstack{SonyAIBORobotSurface2 \\ $\downarrow$ \\ SonyAIBORobotSurface1}}}

& \multirow{4}{*}[0ex]{\shortstack{Full Data}}
& MICN & 74.38 & 80.85 & 77.45 & 74.07 & 76.69 \\
& & TimesNet & 76.37 & 76.62 & 77.14 & 76.30 & 76.61 \\
& & PatchTST & 69.55 & 76.90 & 72.89 & 69.00 & 72.08 \\
& & OneFitsAll & \textbf{79.37} & \textbf{82.30} & \textbf{81.49} & \textbf{79.34} & \textbf{80.62} \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (10\%)}}
& Random init. & 58.51 & 54.26 & 52.51 & 40.88 & 46.53 \\
\cmidrule(lr){3-8}
& & MICN & 62.40 & 61.80 & 61.92 & 61.83 & 61.99 \\
& & TimesNet & 64.23 & 69.14 & 67.07 & 63.82 & 66.07 \\
& & PatchTST & 63.56 & 65.35 & 65.15 & 63.55 & 64.40 \\
& & OneFitsAll & 64.56 & 63.85 & 63.86 & 63.85 & 64.03 \\
& & \myformer & \textbf{91.51} & \textbf{91.36} & \textbf{91.32} & \textbf{91.34} & \textbf{91.38} \\
\cmidrule(lr){2-8}

& \multirow{6}{*}[-1ex]{\shortstack{Few-shot \\ (5\%)}}
& Random init. & 47.09 & 28.55 & 42.45 & 33.61 & 37.94 \\
\cmidrule(lr){3-8}
& & MICN & 56.91 & 52.55 & 50.38 & 39.85 & 49.92 \\
& & TimesNet & 60.23 & 68.97 & 54.02 & 45.82 & 57.26 \\
& & PatchTST & 57.07 & 28.54 & 50.00 & 36.33 & 42.98 \\
& & OneFitsAll & 57.07 & 28.54 & 50.00 & 36.33 & 42.98 \\
& & \myformer & \textbf{85.03} & \textbf{86.45} & \textbf{87.90} & \textbf{85.01} & \textbf{86.09} \\


\hline
\bottomrule
\end{tabular}
\end{small}
\end{threeparttable}
}
\end{table*}

==> tables_brief/classification_full.tex <==
\begin{table}[htbp]
  \caption{Classification (full-data)}\label{tab:brief_classification_full}
  \vskip 0.05in
  \centering
  \resizebox{0.75\columnwidth}{!}{
  \begin{threeparttable}
  \begin{small}
  \renewcommand{\multirowsetup}{\centering}
  \setlength{\tabcolsep}{1pt}
  \begin{tabular}{c|c|c|c|c}
    \toprule
    \hline
    
    \multicolumn{1}{c}{\multirow{2}{*}{Models}} & 
    \multicolumn{1}{c}{\rotatebox{0}{\scalebox{0.8}{\myformer}}} &
    \multicolumn{1}{c}{\rotatebox{0}{\scalebox{0.8}{OneFitsAll}}} &
    \multicolumn{1}{c}{\rotatebox{0}{\scalebox{0.8}{PatchTST}}} &
    \multicolumn{1}{c}{\rotatebox{0}{\scalebox{0.8}{TimesNet}}} \\
    
    \multicolumn{1}{c}{} & 
    \multicolumn{1}{c}{\scalebox{0.8}{(\textbf{ours})}} & 
    \multicolumn{1}{c}{\scalebox{0.8}{\citeyearpar{Zhou2023OneFA}}} & 
    \multicolumn{1}{c}{\scalebox{0.8}{\citeyearpar{Nie2023ATS}}} & 
    \multicolumn{1}{c}{\scalebox{0.8}{\citeyearpar{wu2023timesnet}}} \\
    
    \cline{2-5}
    
    \multicolumn{1}{c}{Metric (\%)} & 
    \scalebox{0.78}{Acc} & \scalebox{0.78}{Acc} & \scalebox{0.78}{Acc} & \scalebox{0.78}{Acc} \\
    
    \hline
    
    \scalebox{0.78}{BeetleFly} &
    \scalebox{0.78}{80.00} &
    \textbf{\scalebox{0.78}{85.00}} &
    \scalebox{0.78}{80.00} &
    \scalebox{0.78}{75.00} \\
    
    % \scalebox{0.78}{BirdChicken} &
    % \scalebox{0.78}{65.00} &\scalebox{0.78}{65.15} &\scalebox{0.78}{65.00} &\scalebox{0.78}{64.91} &\scalebox{0.78}{65.01} &
    % \scalebox{0.78}{75.00} &\scalebox{0.78}{75.25} &\scalebox{0.78}{75.00} &\scalebox{0.78}{74.94} &\scalebox{0.78}{75.05} &
    % \scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &
    % \scalebox{0.78}{65.00} &\scalebox{0.78}{79.41} &\scalebox{0.78}{65.00} &\scalebox{0.78}{60.11} &\scalebox{0.78}{67.38} \\
    
    \scalebox{0.78}{BME} &
    \textbf{\scalebox{0.78}{96.00}} &
    \scalebox{0.78}{93.33} &
    \scalebox{0.78}{88.00} &
    \scalebox{0.78}{92.67} \\
    
    \scalebox{0.78}{CBF} &
    \textbf{\scalebox{0.78}{97.67}} &
    \scalebox{0.78}{87.67} &
    \scalebox{0.78}{89.78} &
    \scalebox{0.78}{93.67} \\
        
    \scalebox{0.78}{Chinatown} &
    \textbf{\scalebox{0.78}{98.96}} &
    \scalebox{0.78}{96.79} &
    \scalebox{0.78}{95.63} &
    \scalebox{0.78}{97.96} \\
    
    \scalebox{0.78}{ChlorineConcentration} &
    \scalebox{0.78}{53.26} &
    \textbf{\scalebox{0.78}{60.05}} &
    \scalebox{0.78}{57.24} &
    \scalebox{0.78}{53.75} \\
    
    % \scalebox{0.78}{CricketX} &
    % \scalebox{0.78}{16.41} &\scalebox{0.78}{7.62} &\scalebox{0.78}{17.46} &\scalebox{0.78}{10.06} &\scalebox{0.78}{12.89} &
    % \scalebox{0.78}{60.77} &\scalebox{0.78}{66.36} &\scalebox{0.78}{61.52} &\scalebox{0.78}{62.31} &\scalebox{0.78}{62.74} &
    % \scalebox{0.78}{67.69} &\scalebox{0.78}{68.66} &\scalebox{0.78}{68.24} &\scalebox{0.78}{68.17} &\scalebox{0.78}{68.19} &
    % \scalebox{0.78}{60.26} &\scalebox{0.78}{60.14} &\scalebox{0.78}{61.06} &\scalebox{0.78}{59.95} &\scalebox{0.78}{60.35} \\
    
    % \scalebox{0.78}{CricketY} &
    % \scalebox{0.78}{13.08} &\scalebox{0.78}{2.81} &\scalebox{0.78}{12.40} &\scalebox{0.78}{4.50} &\scalebox{0.78}{8.20} &
    % \scalebox{0.78}{64.10} &\scalebox{0.78}{67.36} &\scalebox{0.78}{64.00} &\scalebox{0.78}{65.05} &\scalebox{0.78}{65.13} &
    % \scalebox{0.78}{65.38} &\scalebox{0.78}{68.78} &\scalebox{0.78}{65.73} &\scalebox{0.78}{66.55} &\scalebox{0.78}{66.61} &
    % \scalebox{0.78}{65.38} &\scalebox{0.78}{67.00} &\scalebox{0.78}{65.41} &\scalebox{0.78}{65.72} &\scalebox{0.78}{65.88} \\
        
    % \scalebox{0.78}{CricketZ} &
    % \scalebox{0.78}{9.23} &\scalebox{0.78}{0.77} &\scalebox{0.78}{8.33} &\scalebox{0.78}{1.41} &\scalebox{0.78}{4.93} &
    % \scalebox{0.78}{62.82} &\scalebox{0.78}{65.25} &\scalebox{0.78}{62.40} &\scalebox{0.78}{62.73} &\scalebox{0.78}{63.30} &
    % \scalebox{0.78}{68.97} &\scalebox{0.78}{68.57} &\scalebox{0.78}{67.76} &\scalebox{0.78}{67.81} &\scalebox{0.78}{68.28} &
    % \scalebox{0.78}{58.46} &\scalebox{0.78}{58.23} &\scalebox{0.78}{57.29} &\scalebox{0.78}{57.17} &\scalebox{0.78}{57.79} \\
    
    % \scalebox{0.78}{DistalPhalanxOutlineAgeGroup} &
    % \scalebox{0.78}{68.35} &\scalebox{0.78}{50.86} &\scalebox{0.78}{51.69} &\scalebox{0.78}{48.18} &\scalebox{0.78}{54.77} &
    % \scalebox{0.78}{73.38} &\scalebox{0.78}{79.31} &\scalebox{0.78}{68.90} &\scalebox{0.78}{70.69} &\scalebox{0.78}{73.07} &
    % \scalebox{0.78}{74.82} &\scalebox{0.78}{79.76} &\scalebox{0.78}{76.66} &\scalebox{0.78}{75.97} &\scalebox{0.78}{76.80} &
    % \scalebox{0.78}{76.26} &\scalebox{0.78}{78.12} &\scalebox{0.78}{75.77} &\scalebox{0.78}{76.21} &\scalebox{0.78}{76.59} \\
    
    % \scalebox{0.78}{DistalPhalanxOutlineCorrect} &
    % \scalebox{0.78}{58.33} &\scalebox{0.78}{29.17} &\scalebox{0.78}{50.00} &\scalebox{0.78}{36.84} &\scalebox{0.78}{43.59} &
    % \scalebox{0.78}{74.28} &\scalebox{0.78}{77.38} &\scalebox{0.78}{70.50} &\scalebox{0.78}{70.82} &\scalebox{0.78}{73.25} &
    % \scalebox{0.78}{71.74} &\scalebox{0.78}{72.44} &\scalebox{0.78}{68.57} &\scalebox{0.78}{68.85} &\scalebox{0.78}{70.40} &
    % \scalebox{0.78}{76.45} &\scalebox{0.78}{75.78} &\scalebox{0.78}{75.96} &\scalebox{0.78}{75.86} &\scalebox{0.78}{76.01} \\
    
    \scalebox{0.78}{DistalPhalanxTW} &
    \textbf{\scalebox{0.78}{81.22}} &
    \scalebox{0.78}{71.94} &
    \scalebox{0.78}{70.50} &
    \scalebox{0.78}{73.38} \\
        
    % \scalebox{0.78}{Earthquakes} &
    % \scalebox{0.78}{74.82} &\scalebox{0.78}{37.41} &\scalebox{0.78}{50.00} &\scalebox{0.78}{42.80} &\scalebox{0.78}{51.26} &
    % \scalebox{0.78}{75.54} &\scalebox{0.78}{68.06} &\scalebox{0.78}{53.32} &\scalebox{0.78}{50.36} &\scalebox{0.78}{61.82} &
    % \scalebox{0.78}{75.54} &\scalebox{0.78}{71.20} &\scalebox{0.78}{52.38} &\scalebox{0.78}{48.18} &\scalebox{0.78}{61.83} &
    % \scalebox{0.78}{74.82} &\scalebox{0.78}{63.58} &\scalebox{0.78}{55.69} &\scalebox{0.78}{55.19} &\scalebox{0.78}{62.32} \\
    
    \scalebox{0.78}{ECG200} &
    \textbf{\scalebox{0.78}{96.00}} &
    \scalebox{0.78}{91.00} &
    \scalebox{0.78}{86.00} &
    \scalebox{0.78}{89.00} \\
    
    \scalebox{0.78}{ECG5000} &
    \textbf{\scalebox{0.78}{95.53}} &
    \scalebox{0.78}{94.56} &
    \scalebox{0.78}{94.67} &
    \scalebox{0.78}{93.93} \\
    
    \scalebox{0.78}{ElectricDevices} &
    \textbf{\scalebox{0.78}{74.24}} &
    \scalebox{0.78}{62.05} &
    \scalebox{0.78}{66.76} &
    \scalebox{0.78}{69.23} \\
    
    % \scalebox{0.78}{EOGHorizontalSignal} &
    % \scalebox{0.78}{8.29} &\scalebox{0.78}{0.69} &\scalebox{0.78}{8.33} &\scalebox{0.78}{1.28} &\scalebox{0.78}{4.65} &
    % \scalebox{0.78}{42.27} &\scalebox{0.78}{43.44} &\scalebox{0.78}{42.40} &\scalebox{0.78}{41.23} &\scalebox{0.78}{42.34} &
    % \scalebox{0.78}{51.38} &\scalebox{0.78}{52.18} &\scalebox{0.78}{51.36} &\scalebox{0.78}{51.09} &\scalebox{0.78}{51.50} &
    % \scalebox{0.78}{34.25} &\scalebox{0.78}{35.02} &\scalebox{0.78}{34.12} &\scalebox{0.78}{29.72} &\scalebox{0.78}{33.28} \\
    
    % \scalebox{0.78}{EOGVerticalSignal} &
    % \scalebox{0.78}{8.29} &\scalebox{0.78}{0.69} &\scalebox{0.78}{8.33} &\scalebox{0.78}{1.28} &\scalebox{0.78}{4.65} &
    % \scalebox{0.78}{35.08} &\scalebox{0.78}{32.81} &\scalebox{0.78}{34.92} &\scalebox{0.78}{31.87} &\scalebox{0.78}{33.67} &
    % \scalebox{0.78}{47.51} &\scalebox{0.78}{41.46} &\scalebox{0.78}{47.55} &\scalebox{0.78}{43.53} &\scalebox{0.78}{45.01} &
    % \scalebox{0.78}{27.62} &\scalebox{0.78}{26.05} &\scalebox{0.78}{27.39} &\scalebox{0.78}{25.10} &\scalebox{0.78}{26.54} \\
    
    \scalebox{0.78}{FaceAll} &
    \textbf{\scalebox{0.78}{80.00}} &
    \scalebox{0.78}{75.74} &
    \scalebox{0.78}{75.44} &
    \scalebox{0.78}{75.09} \\
    
    \scalebox{0.78}{FaceFour} &
    \scalebox{0.78}{84.09} &
    \textbf{\scalebox{0.78}{90.91}} &
    \scalebox{0.78}{85.23} &
    \scalebox{0.78}{89.77} \\
        
    \scalebox{0.78}{FacesUCR} &
    \textbf{\scalebox{0.78}{95.51}} &
    \scalebox{0.78}{86.15} &
    \scalebox{0.78}{84.83} &
    \scalebox{0.78}{85.07} \\
    
    \scalebox{0.78}{FiftyWords} &
    \textbf{\scalebox{0.78}{80.77}} &
    \scalebox{0.78}{70.33} &
    \scalebox{0.78}{75.16} &
    \scalebox{0.78}{66.15} \\
    
    % \scalebox{0.78}{Fungi} &
    % \scalebox{0.78}{87.63} &\scalebox{0.78}{91.46} &\scalebox{0.78}{87.14} &\scalebox{0.78}{83.95} &\scalebox{0.78}{87.54} &
    % \scalebox{0.78}{86.56} &\scalebox{0.78}{90.73} &\scalebox{0.78}{87.83} &\scalebox{0.78}{86.14} &\scalebox{0.78}{87.81} &
    % \scalebox{0.78}{94.62} &\scalebox{0.78}{95.00} &\scalebox{0.78}{94.37} &\scalebox{0.78}{93.24} &\scalebox{0.78}{94.31} &
    % \scalebox{0.78}{85.48} &\scalebox{0.78}{86.36} &\scalebox{0.78}{86.68} &\scalebox{0.78}{85.75} &\scalebox{0.78}{86.07} \\
    
    \scalebox{0.78}{GunPointAgeSpan} &
    \textbf{\scalebox{0.78}{96.14}} &
    \scalebox{0.78}{89.56} &
    \scalebox{0.78}{89.24} &
    \scalebox{0.78}{94.94} \\
    
    \scalebox{0.78}{GunPointMaleVersusFemale} &
    \textbf{\scalebox{0.78}{99.68}} &
    \scalebox{0.78}{94.62} &
    \scalebox{0.78}{97.47} &
    \scalebox{0.78}{99.05} \\
    
    \scalebox{0.78}{GunPointOldVersusYoung} &
    \textbf{\scalebox{0.78}{98.10}} &
    \scalebox{0.78}{95.05} &
    \scalebox{0.78}{93.65} &
    \scalebox{0.78}{52.38} \\
    
    \scalebox{0.78}{GunPoint} &
    \textbf{\scalebox{0.78}{96.00}} &
    \scalebox{0.78}{92.67} &
    \scalebox{0.78}{76.00} &
    \scalebox{0.78}{94.00} \\
    
    % \scalebox{0.78}{HouseTwenty} &
    % \scalebox{0.78}{64.71} &\scalebox{0.78}{69.05} &\scalebox{0.78}{59.10} &\scalebox{0.78}{55.97} &\scalebox{0.78}{62.21} &
    % \scalebox{0.78}{64.71} &\scalebox{0.78}{63.82} &\scalebox{0.78}{61.58} &\scalebox{0.78}{61.36} &\scalebox{0.78}{62.87} &
    % \scalebox{0.78}{85.71} &\scalebox{0.78}{85.29} &\scalebox{0.78}{85.48} &\scalebox{0.78}{85.38} &\scalebox{0.78}{85.47} &
    % \scalebox{0.78}{63.87} &\scalebox{0.78}{64.97} &\scalebox{0.78}{58.93} &\scalebox{0.78}{56.84} &\scalebox{0.78}{61.15} \\
        
    % \scalebox{0.78}{InsectEPGRegularTrain} &
    % \scalebox{0.78}{47.39} &\scalebox{0.78}{15.80} &\scalebox{0.78}{33.33} &\scalebox{0.78}{21.44} &\scalebox{0.78}{29.49} &
    % \scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &
    % \scalebox{0.78}{83.13} &\scalebox{0.78}{84.74} &\scalebox{0.78}{71.74} &\scalebox{0.78}{72.78} &\scalebox{0.78}{78.10} &
    % \scalebox{0.78}{83.03} &\scalebox{0.78}{84.46} &\scalebox{0.78}{76.61} &\scalebox{0.78}{73.89} &\scalebox{0.78}{79.50} \\
    
    \scalebox{0.78}{InsectEPGSmallTrain} &
    \scalebox{0.78}{83.13} &
    \scalebox{0.78}{75.17} &
    \textbf{\scalebox{0.78}{83.53}} &
    \scalebox{0.78}{83.03} \\
    
    \scalebox{0.78}{InsectWingbeatSound} &
    \textbf{\scalebox{0.78}{69.34}} &
    \scalebox{0.78}{63.03} &
    \scalebox{0.78}{65.56} &
    \scalebox{0.78}{62.58} \\
    
    \scalebox{0.78}{ItalyPowerDemand} &
    \scalebox{0.78}{96.60} &
    \scalebox{0.78}{96.99} &
    \scalebox{0.78}{96.60} &
    \textbf{\scalebox{0.78}{97.18}} \\
    
    % \scalebox{0.78}{Lightning7} &
    % \scalebox{0.78}{53.42} &\scalebox{0.78}{31.01} &\scalebox{0.78}{43.43} &\scalebox{0.78}{35.67} &\scalebox{0.78}{40.88} &
    % \scalebox{0.78}{76.71} &\scalebox{0.78}{83.73} &\scalebox{0.78}{76.43} &\scalebox{0.78}{74.16} &\scalebox{0.78}{77.76} &
    % \scalebox{0.78}{71.23} &\scalebox{0.78}{71.52} &\scalebox{0.78}{69.87} &\scalebox{0.78}{66.31} &\scalebox{0.78}{69.73} &
    % \scalebox{0.78}{76.71} &\scalebox{0.78}{77.11} &\scalebox{0.78}{78.09} &\scalebox{0.78}{75.81} &\scalebox{0.78}{76.93} \\
    
    \scalebox{0.78}{MedicalImages} &
    \textbf{\scalebox{0.78}{84.47}} &
    \scalebox{0.78}{70.53} &
    \scalebox{0.78}{68.55} &
    \scalebox{0.78}{73.03} \\
    
    % \scalebox{0.78}{MiddlePhalanxOutlineAgeGroup} &
    % \scalebox{0.78}{18.83} &\scalebox{0.78}{6.28} &\scalebox{0.78}{33.33} &\scalebox{0.78}{10.56} &\scalebox{0.78}{17.25} &
    % \scalebox{0.78}{64.29} &\scalebox{0.78}{72.26} &\scalebox{0.78}{47.59} &\scalebox{0.78}{49.46} &\scalebox{0.78}{58.40} &
    % \scalebox{0.78}{65.58} &\scalebox{0.78}{72.43} &\scalebox{0.78}{49.12} &\scalebox{0.78}{51.37} &\scalebox{0.78}{59.62} &
    % \scalebox{0.78}{66.23} &\scalebox{0.78}{75.40} &\scalebox{0.78}{48.98} &\scalebox{0.78}{51.02} &\scalebox{0.78}{60.41} \\
    
    % \scalebox{0.78}{MiddlePhalanxOutlineCorrect} &
    % \scalebox{0.78}{57.04} &\scalebox{0.78}{28.52} &\scalebox{0.78}{50.00} &\scalebox{0.78}{36.32} &\scalebox{0.78}{42.97} &
    % \scalebox{0.78}{61.86} &\scalebox{0.78}{68.65} &\scalebox{0.78}{56.19} &\scalebox{0.78}{50.37} &\scalebox{0.78}{59.27} &
    % \scalebox{0.78}{58.42} &\scalebox{0.78}{62.37} &\scalebox{0.78}{52.00} &\scalebox{0.78}{42.24} &\scalebox{0.78}{53.76} &
    % \scalebox{0.78}{85.57} &\scalebox{0.78}{86.07} &\scalebox{0.78}{84.48} &\scalebox{0.78}{84.99} &\scalebox{0.78}{85.28} \\
    
    \scalebox{0.78}{MiddlePhalanxTW} &
    \textbf{\scalebox{0.78}{70.39}} &
    \scalebox{0.78}{60.39} &
    \scalebox{0.78}{62.34} &
    \scalebox{0.78}{61.69} \\
    
    \scalebox{0.78}{MoteStrain} &
    \scalebox{0.78}{88.10} &
    \scalebox{0.78}{87.62} &
    \scalebox{0.78}{85.22} &
    \textbf{\scalebox{0.78}{89.54}} \\
    
    % \scalebox{0.78}{PigAirwayPressure} &
    % \scalebox{0.78}{1.92} &\scalebox{0.78}{0.04} &\scalebox{0.78}{1.92} &\scalebox{0.78}{0.07} &\scalebox{0.78}{0.99} &
    % \scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &
    % \scalebox{0.78}{4.81} &\scalebox{0.78}{4.09} &\scalebox{0.78}{4.81} &\scalebox{0.78}{4.11} &\scalebox{0.78}{4.45} &
    % \scalebox{0.78}{10.58} &\scalebox{0.78}{9.69} &\scalebox{0.78}{10.58} &\scalebox{0.78}{9.21} &\scalebox{0.78}{10.02} \\
    
    % \scalebox{0.78}{PigArtPressure} &
    % \scalebox{0.78}{1.92} &\scalebox{0.78}{0.04} &\scalebox{0.78}{1.92} &\scalebox{0.78}{0.07} &\scalebox{0.78}{0.99} &
    % \scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &
    % \scalebox{0.78}{12.98} &\scalebox{0.78}{11.19} &\scalebox{0.78}{12.98} &\scalebox{0.78}{10.68} &\scalebox{0.78}{11.96} &
    % \scalebox{0.78}{11.06} &\scalebox{0.78}{2.30} &\scalebox{0.78}{11.06} &\scalebox{0.78}{3.60} &\scalebox{0.78}{7.01} \\
        
    % \scalebox{0.78}{PigCVP} &
    % \scalebox{0.78}{1.92} &\scalebox{0.78}{0.04} &\scalebox{0.78}{1.92} &\scalebox{0.78}{0.07} &\scalebox{0.78}{0.99} &
    % \scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &\scalebox{0.78}{00.00} &
    % \scalebox{0.78}{7.21} &\scalebox{0.78}{8.17} &\scalebox{0.78}{7.21} &\scalebox{0.78}{6.97} &\scalebox{0.78}{7.39} &
    % \scalebox{0.78}{9.62} &\scalebox{0.78}{7.88} &\scalebox{0.78}{9.62} &\scalebox{0.78}{6.15} &\scalebox{0.78}{8.32} \\
    
    \scalebox{0.78}{Plane} &
    \textbf{\scalebox{0.78}{99.05}} &
    \scalebox{0.78}{99.05} &
    \scalebox{0.78}{98.10} &
    \scalebox{0.78}{99.05} \\
    
    % \scalebox{0.78}{PowerCons} &
    % \scalebox{0.78}{50.00} &\scalebox{0.78}{25.00} &\scalebox{0.78}{50.00} &\scalebox{0.78}{33.33} &\scalebox{0.78}{39.58} &
    % \scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &
    % \scalebox{0.78}{98.89} &\scalebox{0.78}{98.91} &\scalebox{0.78}{98.89} &\scalebox{0.78}{98.89} &\scalebox{0.78}{98.89} &
    % \scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} &\scalebox{0.78}{100.00} \\
    
    % \scalebox{0.78}{ProximalPhalanxOutlineAgeGroup} &
    % \scalebox{0.78}{48.78} &\scalebox{0.78}{16.26} &\scalebox{0.78}{33.33} &\scalebox{0.78}{21.86} &\scalebox{0.78}{30.06} &
    % \scalebox{0.78}{84.39} &\scalebox{0.78}{56.18} &\scalebox{0.78}{61.30} &\scalebox{0.78}{58.62} &\scalebox{0.78}{65.12} &
    % \scalebox{0.78}{87.80} &\scalebox{0.78}{81.74} &\scalebox{0.78}{79.77} &\scalebox{0.78}{80.67} &\scalebox{0.78}{82.50} &
    % \scalebox{0.78}{85.85} &\scalebox{0.78}{76.64} &\scalebox{0.78}{70.35} &\scalebox{0.78}{72.08} &\scalebox{0.78}{76.23} \\
        
    % \scalebox{0.78}{ProximalPhalanxOutlineCorrect} &
    % \scalebox{0.78}{68.38} &\scalebox{0.78}{34.19} &\scalebox{0.78}{50.00} &\scalebox{0.78}{40.61} &\scalebox{0.78}{48.30} &
    % \scalebox{0.78}{79.73} &\scalebox{0.78}{76.60} &\scalebox{0.78}{76.12} &\scalebox{0.78}{76.35} &\scalebox{0.78}{77.20} &
    % \scalebox{0.78}{78.35} &\scalebox{0.78}{76.20} &\scalebox{0.78}{71.02} &\scalebox{0.78}{72.52} &\scalebox{0.78}{74.52} &
    % \scalebox{0.78}{85.22} &\scalebox{0.78}{88.80} &\scalebox{0.78}{77.51} &\scalebox{0.78}{80.43} &\scalebox{0.78}{82.99} \\
    
    \scalebox{0.78}{ProximalPhalanxTW} &
    \textbf{\scalebox{0.78}{87.44}} &
    \scalebox{0.78}{80.49} &
    \scalebox{0.78}{81.95} &
    \scalebox{0.78}{82.93} \\
    
    % \scalebox{0.78}{ShapesAll} &
    % \scalebox{0.78}{1.67} &\scalebox{0.78}{0.03} &\scalebox{0.78}{1.67} &\scalebox{0.78}{0.05} &\scalebox{0.78}{0.85} &
    % \scalebox{0.78}{72.67} &\scalebox{0.78}{73.93} &\scalebox{0.78}{72.67} &\scalebox{0.78}{71.95} &\scalebox{0.78}{72.80} &
    % \scalebox{0.78}{78.50} &\scalebox{0.78}{79.20} &\scalebox{0.78}{78.50} &\scalebox{0.78}{77.97} &\scalebox{0.78}{78.54} &
    % \scalebox{0.78}{61.00} &\scalebox{0.78}{59.79} &\scalebox{0.78}{61.00} &\scalebox{0.78}{59.34} &\scalebox{0.78}{60.28} \\
    
    % \scalebox{0.78}{SmoothSubspace} &
    % \scalebox{0.78}{33.33} &\scalebox{0.78}{11.11} &\scalebox{0.78}{33.33} &\scalebox{0.78}{16.67} &\scalebox{0.78}{23.61} &
    % \scalebox{0.78}{86.00} &\scalebox{0.78}{85.89} &\scalebox{0.78}{86.00} &\scalebox{0.78}{85.79} &\scalebox{0.78}{85.92} &
    % \scalebox{0.78}{76.67} &\scalebox{0.78}{76.67} &\scalebox{0.78}{76.67} &\scalebox{0.78}{76.20} &\scalebox{0.78}{76.55} &
    % \scalebox{0.78}{96.67} &\scalebox{0.78}{96.78} &\scalebox{0.78}{96.67} &\scalebox{0.78}{96.66} &\scalebox{0.78}{96.69} \\
        
    \scalebox{0.78}{SonyAIBORobotSurface1} &
    \textbf{\scalebox{0.78}{84.19}} &
    \scalebox{0.78}{79.37} &
    \scalebox{0.78}{69.55} &
    \scalebox{0.78}{76.37} \\
    
    \scalebox{0.78}{SonyAIBORobotSurface2} &
    \textbf{\scalebox{0.78}{89.72}} &
    \scalebox{0.78}{86.15} &
    \scalebox{0.78}{85.31} &
    \scalebox{0.78}{81.32} \\
    
    \scalebox{0.78}{SwedishLeaf} &
    \textbf{\scalebox{0.78}{95.20}} &
    \scalebox{0.78}{84.80} &
    \scalebox{0.78}{91.20} &
    \scalebox{0.78}{88.00} \\
    
    % \scalebox{0.78}{Symbols} &
    % \scalebox{0.78}{32.66} &\scalebox{0.78}{12.51} &\scalebox{0.78}{32.60} &\scalebox{0.78}{17.78} &\scalebox{0.78}{23.89} &
    % \scalebox{0.78}{86.83} &\scalebox{0.78}{89.20} &\scalebox{0.78}{86.50} &\scalebox{0.78}{86.40} &\scalebox{0.78}{87.23} &
    % \scalebox{0.78}{86.43} &\scalebox{0.78}{88.34} &\scalebox{0.78}{86.03} &\scalebox{0.78}{86.02} &\scalebox{0.78}{86.70} &
    % \scalebox{0.78}{88.64} &\scalebox{0.78}{90.96} &\scalebox{0.78}{88.29} &\scalebox{0.78}{88.59} &\scalebox{0.78}{89.12} \\
    
    \scalebox{0.78}{SyntheticControl} &
    \textbf{\scalebox{0.78}{100.00}} &
    \scalebox{0.78}{96.33} &
    \scalebox{0.78}{99.00} &
    \scalebox{0.78}{99.67} \\

    % \scalebox{0.78}{ToeSegmentation1} &
    % \scalebox{0.78}{53.51} &\scalebox{0.78}{64.06} &\scalebox{0.78}{50.97} &\scalebox{0.78}{37.27} &\scalebox{0.78}{51.45} &
    % \scalebox{0.78}{65.79} &\scalebox{0.78}{65.70} &\scalebox{0.78}{65.51} &\scalebox{0.78}{65.52} &\scalebox{0.78}{65.63} &
    % \scalebox{0.78}{85.53} &\scalebox{0.78}{85.69} &\scalebox{0.78}{85.32} &\scalebox{0.78}{85.43} &\scalebox{0.78}{85.49} &
    % \scalebox{0.78}{71.49} &\scalebox{0.78}{71.97} &\scalebox{0.78}{70.97} &\scalebox{0.78}{70.95} &\scalebox{0.78}{71.34} \\

    \scalebox{0.78}{ToeSegmentation2} &
    \textbf{\scalebox{0.78}{91.54}} &
    \scalebox{0.78}{84.62} &
    \scalebox{0.78}{83.08} &
    \scalebox{0.78}{84.62} \\

    \scalebox{0.78}{Trace} &
    \scalebox{0.78}{81.00} &
    \scalebox{0.78}{84.00} &
    \scalebox{0.78}{75.00} &
    \textbf{\scalebox{0.78}{92.00}} \\

    % \scalebox{0.78}{TwoPatterns} &
    % \scalebox{0.78}{25.87} &\scalebox{0.78}{6.47} &\scalebox{0.78}{25.00} &\scalebox{0.78}{10.28} &\scalebox{0.78}{16.91} &
    % \scalebox{0.78}{99.48} &\scalebox{0.78}{99.47} &\scalebox{0.78}{99.47} &\scalebox{0.78}{99.47} &\scalebox{0.78}{99.47} &
    % \scalebox{0.78}{99.70} &\scalebox{0.78}{99.70} &\scalebox{0.78}{99.70} &\scalebox{0.78}{99.70} &\scalebox{0.78}{99.70} &
    % \scalebox{0.78}{99.20} &\scalebox{0.78}{99.20} &\scalebox{0.78}{99.21} &\scalebox{0.78}{99.20} &\scalebox{0.78}{99.20} \\

    \scalebox{0.78}{UMD} &
    \textbf{\scalebox{0.78}{99.31}} &
    \scalebox{0.78}{98.65} &
    \scalebox{0.78}{97.92} &
    \scalebox{0.78}{92.50} \\

    % \scalebox{0.78}{UWaveGestureLibraryX} &
    % \scalebox{0.78}{12.62} &\scalebox{0.78}{1.58} &\scalebox{0.78}{12.50} &\scalebox{0.78}{2.80} &\scalebox{0.78}{7.38} &
    % \scalebox{0.78}{78.34} &\scalebox{0.78}{76.55} &\scalebox{0.78}{78.04} &\scalebox{0.78}{76.65} &\scalebox{0.78}{77.39} &
    % \scalebox{0.78}{80.43} &\scalebox{0.78}{79.23} &\scalebox{0.78}{80.21} &\scalebox{0.78}{79.59} &\scalebox{0.78}{79.87} &
    % \scalebox{0.78}{71.55} &\scalebox{0.78}{69.61} &\scalebox{0.78}{71.29} &\scalebox{0.78}{70.12} &\scalebox{0.78}{70.64} \\

    \scalebox{0.78}{UWaveGestureLibraryY} &
    \textbf{\scalebox{0.78}{79.65}} &
    \scalebox{0.78}{67.00} &
    \scalebox{0.78}{70.94} &
    \scalebox{0.78}{63.51} \\

    % \scalebox{0.78}{UWaveGestureLibraryZ} &
    % \scalebox{0.78}{25.57} &\scalebox{0.78}{19.48} &\scalebox{0.78}{25.70} &\scalebox{0.78}{17.02} &\scalebox{0.78}{21.94} &
    % \scalebox{0.78}{69.29} &\scalebox{0.78}{68.37} &\scalebox{0.78}{69.50} &\scalebox{0.78}{67.78} &\scalebox{0.78}{68.73} &
    % \scalebox{0.78}{73.28} &\scalebox{0.78}{72.34} &\scalebox{0.78}{73.45} &\scalebox{0.78}{72.57} &\scalebox{0.78}{72.91} &
    % \scalebox{0.78}{65.27} &\scalebox{0.78}{63.95} &\scalebox{0.78}{65.45} &\scalebox{0.78}{64.28} &\scalebox{0.78}{64.74} \\

    \scalebox{0.78}{Wafer} &
    \textbf{\scalebox{0.78}{100.00}} &
    \scalebox{0.78}{99.58} &
    \scalebox{0.78}{99.37} &
    \scalebox{0.78}{99.53} \\

    \scalebox{0.78}{WordSynonyms} &
    \scalebox{0.78}{56.74} &
    \scalebox{0.78}{58.15} &
    \textbf{\scalebox{0.78}{61.76}} &
    \scalebox{0.78}{56.74} \\

    \hline
    
    \multicolumn{1}{c}{\scalebox{0.78}{{$1^{\text{st}}$ Count}}} & 
    \multicolumn{1}{c}{\scalebox{0.78}{27}} & 
    \multicolumn{1}{c}{\scalebox{0.78}{3}} & 
    \multicolumn{1}{c}{\scalebox{0.78}{2}} & 
    \multicolumn{1}{c}{\scalebox{0.78}{3}} \\
    
    \hline
    \bottomrule
  \end{tabular}
    \end{small}
  \end{threeparttable}
  }
\end{table}
